Decomposing Convolutional Neural Networks into Reusable and Replaceable Modules

Training from scratch is the most common way to build a Convolutional Neural Network (CNN) based model. What if we can build new CNN models by reusing parts from previously build CNN models? What if we can improve a CNN model by replacing (possibly faulty) parts with other parts? In both cases, instead of training, can we identify the part responsible for each output class (module) in the model(s) and reuse or replace only the desired output classes to build a model? Prior work has proposed decomposing dense-based networks into modules (one for each output class) to enable reusability and replaceability in various scenarios. However, this work is limited to the dense layers and based on the one-to-one relationship between the nodes in consecutive layers. Due to the shared architecture in the CNN model, prior work cannot be adapted directly. In this paper, we propose to decompose a CNN model used for image classification problems into modules for each output class. These modules can further be reused or replaced to build a new model. We have evaluated our approach with CIFAR-10, CIFAR-100, and ImageNet tiny datasets with three variations of ResNet models and found that enabling decomposition comes with a small cost (1.77% and 0.85% for top-1 and top-5 accuracy, respectively). Also, building a model by reusing or replacing modules can be done with a 2.3% and 0.5% average loss of accuracy. Furthermore, reusing and replacing these modules reduces CO2e emission by ~37 times compared to training the model from scratch.

==> algocc.tex <==
\begin{algorithm}[ht]
	\caption{Concern Modularization: Channeling (CM-C).}
	\footnotesize
	\label{algo:cmc}
	%\footnotesize
	\begin{algorithmic}[1]
		\Procedure{Channeling($model$, $num\_of\_labels$, $module\_number$, $W$, $B$)}{}\label{algo2:1}
		\If{$module\_number$==0}\label{algo2:2}
		\For{$i=0$ to $|W[0]|$}\label{algo2:3}
		\State temp=[]\label{algo2:4}
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:5}
		\If{$j!=module\_number$}\label{algo2:6}
		\State $temp.add(W[i,j])$\label{algo2:7}
		\State $W[i,j]=0$\label{algo2:8}
		\EndIf
		\EndFor
		\State W[i,1]=Average(temp)\label{algo2:9}
		\EndFor	
		\State $B[1]$=$Average(B[1:num\_of\_labels-1])$\label{algo2:10}
		\State $B[2:num\_of\_labels-1]=0$\label{algo2:11}
		\Else\label{algo2:12}
		\For{$i=0$ to $|W[0]|$}\label{algo2:13}
		\State temp=[]\label{algo2:24}
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:14}
		\If{$j!=module\_number$}\label{algo2:15}
		\State $temp.add(W[i,j])$\label{algo2:16}
		\State $W[i,j]=0$\label{algo2:17}
		\EndIf
		\EndFor
		\State W[i,0]=Average(temp)\label{algo2:18}
		\EndFor	
		\State temp=[]
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:19}
		\If{$j!=module\_number$}\label{algo2:20}
		\State $temp.add(B[j])$\label{algo2:21}
		\State $B[j]=0$\label{algo2:22}
		\EndIf
		\EndFor
		\State $B[0]$=$Average(temp)$\label{algo2:23}
		\EndIf
		\EndProcedure
	\end{algorithmic}    
\end{algorithm}

==> cnnmodularity copy/.git/objects/36/e867d0fa69a440a8a9185204c46ccf1cda1bce <==
xÎÍ
!@aÏTA˜å71ÆŒ0è;kýn´ïð%/÷e™YÄ"Yj
¤4"D®( ë&_rÊQ»'° Ôj¢3F¼pPc‰•tNFY¤äƒóJÛ‹Š•²Æy€ä&‹YàÆÏ>äۃˆå
›<_\g\™NT¶‹Ô¼¶È£²J‰ü]dúïŸëÚß;ž.>˜íIÜ

==> cnnmodularity copy/.git/objects/55/6f476b032e1d74112bbd3f3fa804a66c52fe95 <==
xŽÍ	1=§Š4 ¼¼ü
"– vð'|Y÷à®ÄlÿŠv ÌeSÖÇcšÙìFtŒɶÄN
ÊQ<W
¾!å
[cƒ-"«§t,CGÓ2g
\ŒDטC±?x"
©Õf(ÙÆ}íú&Ë}•EŸúO.³¼†P·³6Á%ώôž<'*ߣ¿bÕæiëPo™‹EÄ

==> cnnmodularity copy/.git/objects/55/a61a8838956b1a9bda73b4b4631f91f1b25d35 <==
xÎÁ
Â0@QΝÂP%qâ¤BŒ€ØÀI¨TZÔºûƒ`Žÿð¥W–çsTp.t_r¬¶%7PÌ(…: ÉÖ#9Š-¥Jó݋W™'±MPlŠIr
Y|¶дØ<
ÓÐHÈv¼ëcYáÆó]DáÊ3œÖ_\FޔUz©û,9"#M0¦+_¢Ê_óǹm ã4ö¡{®«G½

==> cnnmodularity copy/.git/objects/61/142a506b91c8ae544700a20b2dd833d390c981 <==
xŽQjÃ0Dû­SìZV»–,C9BÉ
ÆҪ͇í È¹}LzƒÂü¼ÇLޖåÖItøè͌ʘ (	IÃä‡ì2|QkQσ¶àÝÍÖC¬\u¬af™ÓœÀQŽðÑN£xŸYöþ»5ºbý1ëô•Ní.7<:º}YÙÏä£NÓ <	}rdvù}±Û¿d—±X5CyÒ~/ǎ{´°I

==> cnnmodularity copy/.git/objects/81/24f61b5d1cb11a57470c74f24129d133e003ab <==
x­ŽKnÃ0D»Ö)xúË' HNBJ¢…­@¡7=}ܜ¡«y›y3el[°ÉÉd†"sNN;‡9Зh¨'^=rJÚ8¼	Õ'ïÅ­&¢`³ìÏÆ;jÅæØVËÚۖ™òngkÀ}¿p¡?.'þPÅ]ðU6Z^'­-Ï^¸W0Ѧs7èß:h­Êç´ð?é×.\A}—9êQ¤]½XDY¤

==> cnnmodularity copy/.git/objects/8c/6924b9dccb90ad41ea02547484c41186a1c644 <==
xÎË
Â0€aΙ€òp–bÄNêB´(u÷§'
8þ‡OúÛòzM
ÞÑA»8BŸÂàCÈُØbˆŽXJJÕ×ÑÚÂ-Ž®ˆys—Y!æZyÀœ‹ì"Šo'.ç\-I*Γ5¼ésépçù!¢pãÎý׉We•"Û\ò%aAŠp´ÑZÓ¾‹*áýs]Í
Cy

==> cnnmodularity copy/.git/objects/af/e1cb405aeb7867015d9d09fec1846722b635ac <==
xÎÁ
Â0@QΝ"€»N	!F@làÆôÐ¥.óSÁÿáI?/Ó4šH«ª2ƒ=0!(H¯êi=CK%CW|ß¼¸êl.è1'¢
'‰Y
SQ¡Ì‰"<FéJÛ=—êî<?TÍÝxvçú‹ëÈ«±éIe»8 zÂä½;¶Ô¶Mþ.šþ…÷Ïu]Þ;g«Kó™I\

==> cnnmodularity copy/.git/objects/b6/58ab769638c8bb0c24c7faeacbbbc49a43d448 <==
xíTËnÛ0ìµþŠE€ô¸"õ°Eè!H/9(ŠÜ,(‰Ž…Ò¢KQˆS†ÿÞ¥(:Nœ"ù€B­8³»³CŠ¥%D‹|ñé~Î:¬®Ao8¬¥ò¡iïAñß}£x
;Výb÷¼-áQö
jYõ[ÞjØ)ζ¥à—"s(úŽL³í…n"|°/חš!yº¯jÅVf_I!•ãܬ]aÀ
PbE®@¶âwœyÚ·!÷äN7²BC8"(©R—Ç̕ñ•ì¤(ù}Ӛ!ÿÂ.7z·š|.*627­ÆvߙF4ü䨁X‡ã|\¡¯¥Ô­Ô¼kþð£r½`ʚ'ñ¤þñ¸:Ñ´ßÁ[saMQ¢©ªÞ"ro
Í÷º\›ëh6³>Zk¿€OF·úmkkª§cŽµð%~Ÿ'¼OI'RÎ7'‰¿F	øªuäyVww{uZ9âh'P>Àùßj8bã)yíñ`à°{á@†÷ᬹc"g"çЄ̆ ÈÜ'y(#¹_‰I …‡'Y4ÌHìÉÉ°òBKÐæcG"Ô—ÍC.%c£,phÐ0Ð|$Ó<è̃òt$#ä¦{SC2h c댆j¡#ZäÇÏòg
£EiÐ0Yåy€¢ø:ojHG
~(%‰÷á0l0¡Ñ"†aÃ~å³1=÷SãæÒàL4G
ÞÖîªî6\Ç¿êîÃ?¾†[YsWUÕ+V=NÁa×r»"{ÁPÖb†£`Z³nN)dRVratyÙ¸ÛV¹Û/ìQƒàö/
S1—

==> cnnmodularity copy/.git/objects/bf/e32770f13ca45640eb32e434649aa0271679a0 <==
x]J1"}Î)r¥"t²Ó°ˆGoпº;»Œ™û;¬x_
Šªú ôv½^f®ƒžææž}`ç Ðê€bjJ(}Ñ¢ôÈZ³tçÍי¹†à°Cc'(ZÅOZ«Pë'ì•[üõI¼  «öƒZ1\	Ké¶ HH+"xŸ_·-ðúé>ó;¯ù¼ýš·Ožþ⶿æ2´K~†ôqiú¿Æi¿ÛN?*TL

==> cnnmodularity copy/.git/objects/df/b5a7941a81fcdb296324b2ac0d1768135f9181 <==
xŽË
!@=SÅ4 aÙÄK0v0À {ØOp¶vàñÞË+ë<O
ˆtÐ.T'÷§˜FGÖsô1H)"S-yð¶x×ÌÆ]…ÄeôH'8Ô,V¨ fò9×aL-d7´ÆÎð®ÏµÃ—‡ˆÂ8÷\'~)«œ¤îp#Z"Jp´ÁZS¾‹*Éfßê'
mí3«y‰¿H¥

==> cnnmodularity copy/abstract.tex <==
\begin{abstract}
	% Background - a direct argument about why reuse and replacement is needed.
	% Prior work - what has ESEC/FSE 2020 paper done?
	% Gap - What remains to be done?
	% This work - What are you doing in this work? May be a sentence of insight.
	% Key Results - 
	% to build a new model????
	% describe what the faulty section is????
	Training from scratch is the most common way to build a Convolutional Neural Network (CNN) based model. 
	What if we can build new CNN models by reusing parts from previously build CNN models? 
	% \textbf{(Reuse)} What if there are existing models with all the necessary output classes and more, or a combination of different models that have all the desired classes? 
	What if we can improve a CNN model by replacing (possibly faulty) parts with other parts?
	% (\textbf{Replace}) What if we are building a model because we found that specific output class(es) are not performing as expected. 
	In both cases, instead of training, can we identify the part responsible for each output class (module) in the model(s) and reuse or replace only the desired output classes to build a model?
	Prior work has proposed decomposing dense-based networks into modules (one for each output class) to enable reusability and replaceability in various scenarios. However, this work is limited to the dense layers and based on the one-to-one relationship between the nodes in consecutive layers. Due to the shared architecture in the CNN model, prior work cannot be adapted directly. 
	In this paper, we propose to decompose a CNN model used for image classification problems into modules for each output class. These modules can further be reused or replaced to build a new model. 
	We have evaluated our approach with CIFAR-10, CIFAR-100, and ImageNet tiny datasets with three variations of ResNet models and found that enabling decomposition comes with a small cost (1.77\% and 0.85\% for top-1 and top-5 accuracy, respectively). Also, building a model by reusing or replacing modules can be done with a 2.3\% and 0.5\% average loss of accuracy. 
	Furthermore, reusing and replacing these modules reduces \textbf{$CO_2e$} emission by $\sim$37 times compared to training the model from scratch.
\end{abstract}


==> cnnmodularity copy/algobp.tex <==
%\subsection{Modularizing Concern: Convolution-Based Backtrack (MC-CBB)}
\begin{algorithm}[ht]
	\caption{MC-BI: Modularizing Concern: Backtrack to Input.}
	\footnotesize
	%\footnotesize
	\begin{algorithmic}[1]
		\Procedure{Sliding\_Window\_Mapping($input$, $W$, $pad$, $stride$)}{}
		\State mapping =[], count=0\label{algo4:1}\Comment{Performs the forward pass and map input output nodes}
		\State $temp=zeros_like(input)$\label{algo4:2}
		\State $temp=temp.flatten()$\label{algo4:3}
		\For{$i=0$ to $i=|temp|$}\label{algo4:4}
		\State $temp[i]=i+1$\label{algo4:5}
		\EndFor
		\State $temp=temp.flatten()$\label{algo4:6}
		\State $sliding\_window=sw(temp, W, pad, stride)$\label{algo4:7}
		\For{$i=0$  to $i=|sliding\_window|$}\label{algo4:8}
		\For{$j=0$  to $j=W.length[3]$}\label{algo4:9}
		\State $mapping.add(temp[i][j], count)$\label{algo4:10}
		\EndFor
		\EndFor
		\EndProcedure
		\Procedure{CMBI($input$, $W$, $pad$, $stride$, $B$, $preceeding\_layer$, $deactive\_map$)}{}\label{algo4:11}
		\State $convDepth=depth$\label{algo4:12}
		\State $mapping\_window=Sliding\_Window\_Mapping$($input$, $W$, $pad$, $stride$, $B$)
		\State $source\_mapping=mapping\_window[:0]$\label{algo4:13}\Comment{Input nodes}
		\State $sink\_mapping=mapping\_window[:1]$\label{algo4:14}\Comment{Output nodes}
		\For{each $deactived\_node$ $\in deactive\_map$}\label{algo4:15}
		\State $source$=$source\_mapping$[$sink\_mapping$==$deactived\_node]$\label{algo4:16}
		\State $flag= True$\label{algo4:17}\Comment{Identify the source, where sink is deactive}
		\State $source\_mapping=source\_mapping[source\_mapping]>0]$\label{algo4:18}
		\For {$source\_node$ $\in source\_mapping$}\label{algo4:19}
		\If{$flag==true$}:\label{algo4:20}
		\State $sink\_node$=$sink\_mapping$[$source\_mapping$==$source\_node]$\label{algo4:21}
		\If{$|sink\_node-deactive\_map|>0$}\label{algo4:22}
		\State $flag=false$\label{algo4:23}\Comment{All sinks formed by source are not deactive}
		\EndIf
		\EndIf
		\If{$flag==true$}\label{algo4:24}
		\For{each $source$ $\in source\_mapping$}\label{algo4:25}
		\If{$source$ not $\in deactive\_map$}\label{algo4:26}
		\State $deactive\_map[-1].add(source+1)$\label{algo4:27}\Comment{Update Map}
		\EndIf
		\If{$preceeding\_layer$=="Add"}\label{algo4:28}
		\State $deactive\_map[-2].add(source+1)$\label{algo4:29}\Comment{Update Map}
		\EndIf
		\EndFor
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure
	\end{algorithmic}   
\label{algo:cmfb} 
\end{algorithm}

==> cnnmodularity copy/algocc.tex <==
\begin{algorithm}[ht]
	\caption{Concern Modularization: Channeling (CM-C).}
	\footnotesize
	\label{algo:cmc}
	%\footnotesize
	\begin{algorithmic}[1]
		\Procedure{Channeling($model$, $num\_of\_labels$, $module\_number$, $W$, $B$)}{}\label{algo2:1}
		\If{$module\_number$==0}\label{algo2:2}
		\For{$i=0$ to $|W[0]|$}\label{algo2:3}
		\State temp=[]\label{algo2:4}
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:5}
		\If{$j!=module\_number$}\label{algo2:6}
		\State $temp.add(W[i,j])$\label{algo2:7}
		\State $W[i,j]=0$\label{algo2:8}
		\EndIf
		\EndFor
		\State W[i,1]=Average(temp)\label{algo2:9}
		\EndFor	
		\State $B[1]$=$Average(B[1:num\_of\_labels-1])$\label{algo2:10}
		\State $B[2:num\_of\_labels-1]=0$\label{algo2:11}
		\Else\label{algo2:12}
		\For{$i=0$ to $|W[0]|$}\label{algo2:13}
		\State temp=[]\label{algo2:24}
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:14}
		\If{$j!=module\_number$}\label{algo2:15}
		\State $temp.add(W[i,j])$\label{algo2:16}
		\State $W[i,j]=0$\label{algo2:17}
		\EndIf
		\EndFor
		\State W[i,0]=Average(temp)\label{algo2:18}
		\EndFor	
		\State temp=[]
		\For{$j=0$ to  $num\_of\_labels$}\label{algo2:19}
		\If{$j!=module\_number$}\label{algo2:20}
		\State $temp.add(B[j])$\label{algo2:21}
		\State $B[j]=0$\label{algo2:22}
		\EndIf
		\EndFor
		\State $B[0]$=$Average(temp)$\label{algo2:23}
		\EndIf
		\EndProcedure
	\end{algorithmic}    
\end{algorithm}

==> cnnmodularity copy/algoci.tex <==
%\section{Concern Identification}
\begin{algorithm}[ht]
	\caption{Concern Identification (CI).}
	\footnotesize
	\label{algo:concern}
	%\footnotesize
	\begin{algorithmic}[1]
		\Procedure{Initialization($model$)}{}\label{algo1:1}
		\State $convW$, $convB$ =[]\label{algo1:2}
		\For{each layer $\in model$}\label{algo1:3}\Comment{Retrieve the weight and bias}
		\If{$layer_{type}$=="Convolution"}\label{algo1:4}
		\State $convW.add(layer.Weight); convB.add(layer.Bias);$
		\Else \If{$layer_{type}$=="Dense"}\label{algo1:5}
		\State  $denseW.add(layer.Weight); denseB.add(layer.Bias);$\label{algo1:6}
		\EndIf
		\EndIf
		\EndFor
		\State \Return $convW, convB, denseB, denseW$\label{algo1:7}
		\EndProcedure
		\Procedure{CILayer ($model$, $input$, $convW_{Layer}$,\label{algo1:8} $convB_{Layer}$,  $convMap_{Layer}$, $pad$=$with$, $Stride$=$1$, $first$=$False$)}{}
		\State $I$=$input$\label{algo1:9}
		\State $sliding_{w}$=$procSliding(I$, $pad$, $(Stride$, $Stride))$\label{algo1:10} \Comment{Sliding window}
		\State $Output$=$sliding_{w}*convW_{Layer}$ + $convB_{Layer}$\label{algo1:11} 
		\State $flatOutput$=$flatten(Output)$\label{algo1:12} \Comment{Convert into an 1-D array}
		\For{$j=0$ to $j=|flatOutput|$}\label{algo1:13} 
		\If{$first$}\label{algo1:14}
		\If{$flatOutput[j]$<=0}\label{algo1:15}\Comment{Identify the inactive nodes}
		\State $convMap_{Layer}.add(j)$\label{algo1:16}
		\EndIf
		\Else \Comment{Remove the inactive node if it is active for other inputs}
		\If{$j\in convMap_{Layer}$ }\label{algo1:17}
		\If{$flatOutput[j]$>0}\label{algo1:18}
		\State $index$=$findIndex(flatOutput, j)$\label{algo1:19}
		\State temp=[]\label{algo1:20}
		\For{$k=0$ to $k=convMap_{Layer}$}\label{algo1:21}
		\If{$k!=index$}\label{algo1:22}
		\State $temp.add(convMap_{Layer}[k])$\label{algo1:23}
		\EndIf
		\EndFor
		\State $convMap_{Layer}$=$temp$\label{algo1:24}
		\EndIf
		\EndIf
		\EndIf
		\EndFor
		\State \Return $convMap_{Layer}$, $Output$\label{algo1:25}
		\EndProcedure
		\Procedure{CI ($model$, $input, convMap$)}{}
		
		\State $convW, convB, denseB, denseW$=$initialization(model)$\label{algo1:26}
		\For{each $layer \in model$}\label{algo1:27}\Comment{Perform CI for all the layers}
		\State count=0\label{algo1:28}
		\If{$layer_{type}$==$``Convolution"$}\label{algo1:29}
		\State convMap[count], output = CILayer(($model$, $input$, $convW[count]$, $convB[count]$,  $convMap[count]$, $pad$=$layer_{pad}$, $Stride$=$layer_{stride}$))\label{algo1:30}
		\EndIf
		\If{$layer_{type}$=$``BatchNormalization"$}\label{algo1:31}
		\State output = BatchNorm(($model$, $Gamma$))\label{algo1:32}
		\EndIf
		\If{$layer_{type}$==$``AveragePooling"$}\label{algo1:33}
		\State output = AvgPool(($model$, $Pool_{Size}$))\label{algo1:34}
		\EndIf
		\If{$layer_{type}$=$``MaxPooling"$}\label{algo1:35}
		\State output = MaxPool(($model$, $Pool_{Size}$))\label{algo1:36}
		\EndIf
		\If{$layer_{type}$=$``Add"$}\label{algo1:37}
		\State output = input+$Previous_{input}$\label{algo1:38} \Comment{Add both the layers that are merged}
		\EndIf
		\If{$layer_{type}$=$``Dense"$}\label{algo1:39}
		\State output = denseMod($model$, $input$, $indicator$=$False$, $denseW[count]$, $denseB[count]$)\label{algo1:40}\Comment{Apply dense-based CI}
		\EndIf
		\If{$layer_{type}$=$``Flatten"$}\label{algo1:41}
		\State output = flatten($input$)\label{algo1:42} \Comment{Apply flatten-based CI}
		\EndIf
		\State $input$=$output$
		\EndFor
		\EndProcedure
	\end{algorithmic}    
\end{algorithm}

%Concern Identification (CI) involves identifying the section of the CNN model responsible for the single output class. In this process, we remove nodes and edges in the model. In traditional CNN models for image-classification,  both convolution and dense layers have the notion of node and edges, and we discuss the concern identification approaches for both the layers. In this paper, we use concerned and non-concerned as terminologies that represent the input belonging to the output class for which module has been created and all the other output classes, respectively. Compared to the prior work on decomposition, we identify the inactive output nodes at each layer.
%For dense, we used the dense-based approach for identifying the concerns as discussed by Pan~\etal~\cite{pan2020decomposing}.



==> cnnmodularity copy/algodbp.tex <==
\begin{algorithm}[ht]
	\caption{MC-BLN: Modularizing Concern: Backtrack to Last Convolutional Layer (MC-BLN).}
	\footnotesize
	\label{algo:cmdbb}
	%\footnotesize
	\begin{algorithmic}[1]
		\Procedure{CMBLN($model$, $num\_of\_labels$, $module\_class$, $UpdatedW$, $UpdatedB$)}{}\label{algo3:1}
		\State $temp$, $tempL$, $tempPool=[]$\label{algo3:2} \Comment{UpdateW: Weight for Dense Layers}
		\State $DenseLength=|UpdatedW|$\label{algo3:3}\Comment\Comment{UpdateB: Bias for Dense Layers}
		\For{$i=0$ to $i=UpdatedW[DenseLength-1][0]$}\label{algo3:4}
		%\If{$module\_class==0$}\label{algo3:5}\Comment{First output class is concerned class}
		\If{UpdatedW[DenseLength-1][i,$v_{uc}$]<=-$\delta$ and UpdatedW[DenseLength-1][i,$v_c$]>=+$\delta$}\label{algo3:6} 
		\State $temp.add(i)$\label{algo3:7} \Comment{$v_c$: concerned nodes, $v_{uc}$: unconcerned nodes}
		\EndIf
		\EndFor
		\State $tempL.add(temp)$\label{algo3:10}
		\For{$i=DenseLength-1|$ to $i=0$}\label{algo3:11}\Comment{Backtrack till the first Dense}
		\State $temp=[]$\label{algo3:12}
		\For{$j=0$ to $j=UpdatedW[i-1][0]$}\label{algo3:13}
		\If{$j \in tempL[i]$}\label{algo3:14}
		\If{UpdatedW[i-1][j:,]<=-$\delta$}\label{algo3:15}
		\State $temp.add(i)$\label{algo3:16}\Comment{Add nodes that are only connected with $v_{nc}$}
		\EndIf
		\EndIf
		\EndFor
		\State $tempL.add(temp)$\label{algo3:17}
		\EndFor
		\For{$i \in tempL[|tempL-1|]$}\label{algo3:18}
		\For{$j=0$ to $j=i*poolsize^2+j$}\label{algo3:19}\Comment{Convert to pooling layer}
		\If{Layer-1=="Convolution"}\label{algo3:20}
		\If{j not $\in$ convMap[depth]}\label{algo3:21}
		\State convMap[depth].add(j)\label{algo3:22} \Comment{Update convolution layer map}
		\EndIf
		\EndIf
		\If{Layer-1=="Add"}\label{algo3:23} \Comment{Update two convolution layer maps}
		\If{j not $\in$ convMap[depth]}\label{algo3:24}
		\State convMap[depth].add(j)\label{algo3:25}
		\EndIf
		\State depthAdd2=Add.Input2\label{algo3:26}
		\If{j not $\in$ convMap[depthAdd2]}\label{algo3:27}
		\State convMap[depthAdd2].add(j)\label{algo3:28}
		\EndIf
		\EndIf
		\EndFor
	
		\EndFor
		\EndProcedure
	\end{algorithmic}    
\end{algorithm}

==> cnnmodularity copy/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
In this paper, we introduce decomposition in convolutional networks and transform a trained model into smaller components or modules. We used a data-driven approach to identify the section in the model responsible for a single output class and convert that into a binary classifier. 
Modules created from the same or different datasets can be reused or replaced in any scenario if the input size of the modules is the same. We found that decomposition involves a small cost of accuracy. However, both intra-dataset reuse and replaceability increase the accuracy compared to the trained model. Furthermore, enabling reusability and replaceability reduces $CO_2e$ emission significantly. For this work, we omit the heterogeneous inputs (the input size for modules are not the same) while reusing and replacing modules, and it will be a good 
research direction for the future to study how an interface could be built around the modules to take different types of inputs.

==> cnnmodularity copy/dataset.tex <==
\section{Dataset and Model Descriptions}
\paragraph{Datasets} We evaluate our proposed approach based on three widely used and well-vetted datasets.

\noindent\textbf{CIFAR-10~\cite{krizhevsky2009learning}:} This dataset comprises of 3-D images of different objects. It has 10 output classes, and the dataset is divided into training and testing datasets. The training dataset has 50,000 images and the testing dataset has 10,000 images. The number of examples for each class is equally distributed. The output classes are airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. Each of the images is of size (32, 32, 3), where the length, width, and color channels are 32, 32 pixels, and three dimensions, respectively.

\noindent\textbf{CIFAR-100~\cite{krizhevsky2009learning}:} This dataset has 100 output classes. This is widely used to evaluate CNN-based studies due to the complexity of the dataset. Here, there are 50,000 training images and 10,000 testing images. There are 20 different types of images in this dataset, and for each type, there are 5 varieties of images are there. For instance, one of twenty superclasses is the aquatic animal, and within that class, we have beaver, dolphin, otter, seal, and whale. The image size is similar to the CIFAR-10.

\noindent\textbf{ImageNet-200~\cite{deng2009imagenet}:} This dataset is very popular and widely use to measure the scalability of CNN-based applications. Unlike the previous two datasets, the total number of output classes is 200. ImageNet dataset has been designed to help the computer vision-related task in machine learning. This dataset has 80,000+ nouns (name of the class), and for each class, there are at least 500 images associated with it. This dataset has been used in training models in real-life scenarios. However, due to the complexity of the dataset, a smaller dataset specially intended for research purposes with similar complexity has been made public. This dataset (ImageNet-tiny) comprises 200 types of images. The training dataset has 100000 images, and the testing has 10000 images. There are 3 different variations of the dataset, where the length and width of the images are 224, 64, and 32. In our experiments, we used the 64 version of the dataset to reduce the time-complexity of training such networks and have an experimental dataset that is different from CIFAR-10 and CIFAR-100 in terms of the image size. 
\paragraph{Models} In this study, we used the ResNet models to evaluate our proposed approach. There are multiple blocks present in a ResNet model, and each block consists of convolution, add, and activation layers. There are two versions of ResNet, the original version, where there is a stack of convolution, add, and batch normalization layers are put together to form a residual block, and finally, those residual blocks build the network. In the second version, the residual block is modified to form a bottleneck layer with convolution, add, and batch normalization. We performed our evaluation against the first version of the network for simplicity and to reduce the training time and resources. Each such version can either have a batch normalization layer or not, as described in the original paper. Since batch normalization is only used to train and does not participate in the prediction, we chose the model without batch normalization to reduce the training time as some of our experiments include training models multiple times. We used ResNet-20, ResNet-32, and ResNet-56, where 3, 5, and 9 residual blocks are present with 21, 33, and 57 convolution layers, respectively. The accuracy reported in this study is different from the original paper because we re-trained the model from scratch with 200 epochs.

The code can be accessed at.

==> cnnmodularity copy/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% Background .
% Prior works
% Gap - What remains to be done?
% This work - What are you doing in this work?
% Key Results - 
Deep learning is increasingly being used for image segmentation, object detection, and similar computer vision tasks. With the need for bigger and complex datasets, the size and complexity of models also increase. Often, training a model from scratch needs several hours or even days. 
To ease the training process, layer architecture~\cite{sun2018resinnet, luo2017thinet}, transfer learning~\cite{torrey2010transfer, tan2018survey}, one-shot learning~\cite{vinyals2016matching, rezende2016one}, few-shot learning~\cite{sung2018learning, sun2019meta, lifchitz2019dense, wertheimer2019few}, etc., have been introduced. With these techniques, model structure, parameters can be reused for building a model for similar or different problems. However, in all cases, retraining is needed. Also, there may be scenarios, as shown in Figure \ref{fig:overview}, where a faulty section of the network needs to be amputated or replaced. Now, suppose we can decompose a Convolutional Neural Network (CNN) into smaller components (modules), where each component can recognize a single output class. In that case, we can reuse these components in various settings to build a new model, remove a specific output class, or even replace an output class from a model without retraining. In the past, modular networks~\cite{andreas2016neural, hu2017learning, ghazi2019recursive}, capsule networks~\cite{hinton2000learning, sabour2017dynamic}, etc., have been studied to train the network and incorporate memory into the learning process. But, these modules are not created for enabling reusability and replaceability. 
As others have noted~\cite{pan2020decomposing}, 
there are strong parallels between deep neural network development now and software development
before the notion of decomposition was introduced~\cite{dijkstra1982role, parnas1972criteria, tarr1999n}, and developers wrote monolithic code that can be reused or replaced as easily. 

Recently, decomposition has been used to enable reuse and replacement in dense-based networks~\cite{pan2020decomposing}. 
This work shows that decomposed modules can be reused or replaced in various scenarios. However, this work focused on dense-based networks and did not explore a more complex set of deep learning techniques, e.g., convolutional neural networks. This work~\cite{pan2020decomposing} relies on the dense architecture of the models, where nodes and edges (weight and bias) have a one-to-one relationship. In contrast, edges in CNN are shared among all the input and the output nodes.
\begin{figure*}%
	\centering
	\footnotesize
	\subfloat{\includegraphics[, width=1.0\linewidth]{overview.pdf}}%
	\qquad
	\subfloat{\input{tbMotiv.tex}}
	\caption{How Decomposing a Convolution Neural Network into Modules Can Help Solve a Real-life Problem.}%
	\label{fig:overview}%
\end{figure*}

In this paper, we propose an approach to decompose a CNN model used for image classification into modules, in which each module can classify a single output class. Furthermore, these modules can be reused or replaced in different scenarios. In Figure \ref{fig:overview}, we illustrate an issue faced by users while using the Google Photo app. We show how Google has resolved the problem and how replacing and reusing decomposed modules can be applied. 
In the past, Google Photo App tagged a black woman as a gorilla~\cite{verge}.
To resolve this issue, Google decided to remove the output class ``Gorilla'' 
by suppressing the output label~\cite{verge}. Precisely, they have suppressed the output for ``Chimpanzee'', ``Monkey'', ``Chimp'', etc. Though the problem can be temporarily solved by suppressing the output label, to fix the model, one needs to retrain the model. We propose four different solutions based on reusing and replacing decomposed modules. We discuss each approach, its pros, cons, and illustrate how retraining the model can be avoided. The code and other artifacts are made available~\footnote{https://github.com/rangeetpan/Decomposition}.

The key contributions of our work are the following: 

\begin{itemize}
	\item We introduce a technique to decompose a CNN model into modules, one module per output class.  
	\item We describe an approach for reusing these decomposed modules in different scenarios to 
	build models for new problems.
	\item We replace a part of the model with decomposed modules.
	\item We evaluate our approach against the $CO_2e$ consumption of models created from scratch and reusing or replacing decomposed modules.
\end{itemize}
%1) decomposing CNN models into modules, 2) enabling reusability and replaceability, and 3) evaluate the $CO_2e$ emission for both decomposing and training-based approaches. 

\textbf{Results-at-a-glance. }Our evaluation suggests that decomposing a CNN model can be done with a little cost (-1.77\% (top-1) and -0.85\% (top-5)) compared to the trained model accuracy. Reusing and replacing modules can be done when the modules belong to the same datasets (reusability: +2.5\%, replaceability: +0.7\% (top-1) and +1.0\% (top-5)) and the different datasets (reusability: -7.63\%, replaceability: +2.5\% (top-1) and -7.0\% (top-5)). Furthermore, enabling reusability and replaceability reduce $CO_2e$ emission by 37 times compared to training from scratch.

\textbf{Outline.} In \S\ref{sec:related} we describe the related work. Then in \S\ref{sec:methodology}, we discuss our approach to decompose a CNN model into modules. In \S\ref{sec:results}, we answer three research questions to evaluate the cost of decomposition, the benefit of reusing or replacing the modules, and the resource consumption. Lastly, in \S\ref{sec:conclusion}, we conclude.
\begin{figure*}[htp]
	\centering
	\includegraphics[, width=1\linewidth]{approach.pdf}
	\caption{High-level Overview of Our Approach. Inactive nodes are denoted by black boxes.}
	\label{fig:approach}
\end{figure*}

==> cnnmodularity copy/macro.tex <==
%\usepackage[table]{xcolor}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{multirow}
\usepackage{booktabs} % For formal tables
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{caption}
%\usepackage{subcaption}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage[
font=footnotesize % or small or scriptsize
]{subfig}
%\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{listings}
\usepackage{color, colortbl}
\usepackage{balance} % to balance the bibliography
\usepackage{lscape}
\usepackage{hyperref}
\usepackage{xspace}
\usepackage{framed}
\usepackage{syntax}
%\usepackage{hyperref}
%\usepackage{mdframed}
%\usepackage[framemethod=TikZ]{mdframed}
\usepackage{soul}
\usepackage{flushend}
\usepackage[tikz]{bclogo}
% loads also »colortbl«
\usepackage{makecell}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{Gray}{gray}{0.1}
%\rowcolors{2}{gray!25}{white}
\lstdefinestyle{mystyle}{
	backgroundcolor=\color{backcolour},   
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\scriptsize,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	numbersep=5pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}



\lstdefinelanguage{Pythonna}{%
	language     = python,
	morekeywords = {to_categorical, flow_from_directory,pad_sequences,load_image},
	morecomment=[f][\color{diffstart}]{@@},
	morecomment=[f][\color{diffincl}]{+\ },
	morecomment=[f][\color{diffrem}]{-\ }	
}

\lstdefinestyle{customc}{
	belowcaptionskip=1\baselineskip,
	breaklines=false,
	frame= single,
	%numbers = left,
	breaklines = true,
	xleftmargin=\parindent,
	language= Pythonna,
	showstringspaces=false,
	basicstyle=\footnotesize\ttfamily,
	keywordstyle=\bfseries\color{green!40!black},
	commentstyle=\itshape\color{purple!40!black},
	identifierstyle=\color{blue},
	stringstyle=\color{codegreen},
	backgroundcolor=\color{gray!4}
}


\lstset{style=customc}
\newcommand{\change}[1]{{\color{blue!80!white}\textbf{}~#1}\xspace}
%\usepackage{pdflscape}
\newcommand{\centerhfill}[1][\quad]{\hspace{\stretch{0.5}}#1\hspace{\stretch{0.5}}}
\graphicspath{{./figures/}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\fignref}[1]{Figure~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\secnref}[1]{\S\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\theref}[1]{Theorem~\ref{#1}}
\newcommand{\lineref}[1]{line~\ref{#1}}
\newcommand{\linesref}[2]{lines~\ref{#1}-\ref{#2}}
\newcommand{\linerefNum}[1]{\ref{#1}}
\newcommand{\footnoteref}[1]{$^{\ref{#1}}$}
\newcommand{\commitcount}{100\xspace}
\newcommand{\totalcommit}{500\xspace}
\newcommand{\etal}{{\em et al.}\xspace}
\newcommand{\albert}{\textit{ALBERT}\xspace}
\newcommand{\conv}{\textit{Convolution}\xspace}
\newcommand{\bart}{\textit{Bart}\xspace}
\newcommand{\bert}{\textit{Bert}\xspace}
\newcommand{\ctrl}{\textit{CTRL}\xspace}
\newcommand{\gpt}{\textit{GPT-2}\xspace}
\newcommand{\roberta}{\textit{RoBERTa}\xspace}
\newcommand{\tf}{\textit{T5}\xspace}
\newcommand{\txl}{\textit{Transformer-XL}\xspace}
\newcommand{\xlnet}{\textit{XLNET}\xspace}
\newcommand{\xlm}{\textit{XLM}\xspace}

\newcommand{\code}[1]{{\texttt{\footnotesize{#1}}\xspace}}

\newcommand{\sof}{\textit{Stack Overflow}\xspace}
\newcommand{\caffe}{\textit{Caffe}\xspace}
\newcommand{\ho}{\textit{H2O}\xspace}
\newcommand{\keras}{\textit{Keras}\xspace}
\newcommand{\mahout}{\textit{Mahout}\xspace}
\newcommand{\mllib}{\textit{MLlib}\xspace}
\newcommand{\scikit}{\textit{scikit-learn}\xspace}
\newcommand{\tensor}{\textit{Tensorflow}\xspace}
\newcommand{\theano}{\textit{Theano}\xspace}
\newcommand{\torch}{\textit{Torch}\xspace}
\newcommand{\weka}{\textit{Weka}\xspace}
\newcommand{\gh}{\textit{GitHub}\xspace}
\newcommand{\paddle}{\textit{paddle}\xspace}
\newcommand{\wa}[1]{{\color{orange!80!white}\textbf{Who to work on:}~#1}\xspace}
\newcounter{rqs}
\stepcounter{rqs}

\newcommand{\sbug}{\textit{320}\xspace}
\newcommand{\gbug}{\textit{347}\xspace}
\newcommand{\qn}[1]{{\bf{RQ\arabic{rqs}: } \em #1}
	\stepcounter{rqs}
}

\newcounter{NumObservations}
\stepcounter{NumObservations}
\definecolor{shadecolor}{rgb}{.9,.9,.9}




\newcommand{\findingold}[1]{%
	\begin{mdframed}[
		backgroundcolor= gray!10,
		linewidth=.2pt,
		linecolor = gray!110,
		roundcorner=2pt,
		innertopmargin=2pt,
		innerbottommargin=0pt,
		innerrightmargin=4pt,
		innerleftmargin=2pt,
		leftmargin = 0pt,
		rightmargin = 0pt]%
		\noindent{\textbf{Finding \arabic{NumObservations}}: \em #1} \\
	\end{mdframed}%
	\stepcounter{NumObservations}
}


\newcommand{\findingsold}[1]{
	
	\begin{shaded}
		\vspace{-.85em}
		%\hspace{1.5em}
		\textit{{\bf{Finding \arabic{NumObservations}}}: #1.}\\
		\vspace{-1.75em}
	\end{shaded}
	\stepcounter{NumObservations}	
}


\newcommand{\finding}[1]{
	\begin{bclogo}[couleur= blue!5, epBord= 1, arrondi=0.1, logo=\bclampe,marge= 2, ombre=true, blur, couleurBord=blue!60, tailleOndu=3, sousTitre ={\em #1}]{Finding \arabic{NumObservations} $\Rightarrow$ } 
		
	\end{bclogo}
	\stepcounter{NumObservations}
}


==> cnnmodularity copy/methodology.tex <==

\section{Approach}
\label{sec:methodology}
In this section, we provide an overview of our approach for CNN model decomposition. We discuss the challenges in general. We also discuss each step of decomposing a CNN model into modules.

Figure \ref{fig:approach} shows the steps for decomposing a CNN model into modules. Our approach starts with the trained model and identifies the section in the CNN that is responsible for a single output class (Concern Identification). Since we remove nodes for all non-concerned output classes, the identified section acts as a single-class classifier. To add the notion of the negative output classes, we add a limited section of the inputs from unconcerned output classes (Tangling Identification). Finally, we channel the concerns to create a module(s) (Concern Modularization). In the example, we show the decomposition of the module for the output class A. Here,  a model trained to predict four output classes has been decomposed into four modules. Each one is a binary classifier that recognizes if an input belongs to the output class. 
In this paper, we use \textit{concerned} and \textit{unconcerned} as terminologies that represent the input belonging to the output class for which module has been created and all the other output classes, respectively.
For example, in Figure~\ref{fig:approach}, we show a module that is responsible for identifying output class $A$. For that module, output class $A$ is the concerned output class, and other output classes, e.g., $B$, $C$, and $D$, are the unconcerned classes.
\subsection{Challenges}
\label{subsec:challenges}
In the prior work on decomposing dense-based models, 
modules were created by removing edges. There, the value of the node has been computed. If it is $\le$0, then all incoming and outgoing edges are removed.
In a typical dense-based model, the first layer is a flatten layer that converts an input into a single-dimensional representation. From there, one or more dense layers are attached sequentially. In each such dense layer, nodes are connected with two different edges, 1) an edge that connects with other nodes from the previous layer (weight) and 2) a special incoming edge (bias). However, for a \conv layer, this is not the case. 
%In \conv layer, each weight is shared by all the nodes (we can alternatively call them cells) in the output. 
Figure \ref{fig:cnn} illustrates a traditional \conv layer. In that figure, on the left side, we have input nodes. Weight and bias are shown in the middle, and finally, on the right side, we have the output nodes. Each node in the input is not directly connected with the weight and bias, rather a set of nodes (sliding window) are chosen at a time as the input, and the output is computed based on that. The weight and bias are the same for all the input blocks. Due to these differences in the underlying architecture of a \conv layer, the dense-based decomposition approach could not be applied to a \conv layer directly. In the next paragraphs, we discuss each of such challenges.
\begin{figure}
	\centering
	\includegraphics[, width=1\linewidth]{cnn.pdf}
	\caption{Architecture of a Convolutional Layer. }
	\label{fig:cnn}
\end{figure}

\textbf{Challenge 1: Shared Weight and Bias.} 
The removal of edges in dense-based layers has been done to forcing the value of the nodes that are not needed to be 0 and eventually remove them from the decision-making process in the module. This approach is possible in dense layers because there is a one-to-one relationship between two nodes that belong to subsequent layers. If we remove a part of the weight and bias for one node in the  \conv layer, the weight and the bias will be turned off for all other nodes as well, and there will not be any output produced. 

\textbf{Challenge 2: Backtracking.} The prior work  channels the concerns to convert the module into a binary classification problem. However, before channeling the output nodes, a backtracking approach has been applied that starts with removing nodes at the last hidden layer that are only connected to the unconcerned nodes at the output layers and backtrack to the first hidden layer. However, the same approach cannot be directly applied to the CNN models due to the differences in the architecture of the convolutional layers and other supporting layers, e.g., \textit{Pooling}, \textit{Merge}.

\textbf{Challenge 3: Loss of Accuracy in Inter-Dataset Scenarios.} Prior work evaluated their approach by reusing and replacing modules that belong to different datasets. It has been found that such scenarios involve a non-trivial cost.
%In the prior work, the inter-dataset reuse and replacement scenarios are associated with a non-trivial cost. 
Since these modules involved in the reuse and replace scenario do not belong to the same datasets, they are not programmed to distinguish between them. To remediate the cost, we propose a continuous learning-based approach that enables retraining of the decomposed modules.


==> cnnmodularity copy/motivation.tex <==
\section{Motivation}
\label{sec:motivation}
\begin{figure*}[!ht]
	\includegraphics[, width=1\linewidth]{overview.pdf}
	\caption{How Decomposing a Convolution Neural Network can Help Solving a Real-life Problem.}
	\label{fig:overview}
\end{figure*}
Decomposing a convolutional neural network into modules can help to achieve various real-life scenarios. Because of the complex architecture and the massive size, retraining a model from scratch is not always feasible. Instead of building a new model, we propose utilizing parts from the already trained model and reusing or replacing them based on different scenarios. First, we describe one such requirement, where replacing a section of the model (module) with another (module) can be done with no or little retraining. Then, we describe how reusing these modules can be done.

In Figure \ref{fig:overview}, we have shown a real-life example, where Google Photo App tagged a black woman as a gorilla. To resolve this issue, Google has decided to remove the output class ``Gorilla'' by suppressing the output label. In fact, they have suppressed labels for ``Chimpanzee'', ``Monkey'', ``Chimp'', etc~\cite{verge}., from the output of the convolutional neural network. Though the problem can be temporarily solved by suppressing the output label, to fix the model, one needs to retrain from scratch, which requires both high-computational and time-related resources. Instead of the prior approach, we propose three different solutions that reuse and replace modules from the trained model. We will discuss each of such approaches and their pros and cons and illustrate how retraining the model can be avoided. 

First, we decompose the faulty convolution neural network into modules for each output class. For instance, we have one module for each output class that classifies whether an input belongs to the output class, for which the module has been created, or not. In this example, our goal is to replace the faulty part or module responsible for classifying gorilla with a working module for the same. If we have another working model that is either trained with the same dataset or a subset of the dataset, we will decompose that working model into modules. The working model needs to have the gorilla and person output label, and that model should not exhibit the behavior present in the faulty model. Then, we can replace the faulty gorilla module with the working gorilla module, and a composed version of the decomposed modules can be sent to production. However, the drawback of this approach is the availability of such models. Training a model with a large dataset needs heavy computational resources and a non-trivial amount of time.

Second, we decompose the faulty model into modules. Moreover, we train a new model with a person and gorilla and validate that the trained model does not demonstrate faulty behavior. We decompose the newly trained model into two modules and replace the faulty gorilla module with the new decomposed gorilla module. In this scenario, decomposition can not alone solve the problem. However, the decomposition bundled with the traditional training could help in this situation. Also, training the small model requires less resources.

Third, we decompose the faulty model into modules and remove the gorilla module from the collection. In this scenario, there is no cost of retraining involved. However, using this approach, the actual problem of faulty classification has not been addressed. This solution is similar to what Google proposed, but instead of suppressing the label, we remove the module. The pros in this situation are that for other primates (``Chimpanzee'', ``Monkey'', ``Chimp'', etc.), we can remove the modules easily, whereas, for the other two techniques, we need to have models with those output classes or train a small network for them. 

We can also reuse the person and gorilla module from a working model without the faulty behavior and predict any input classified as a person or gorilla using the faulty model to verify it further. Here, instead of replacing the faulty parts, we reuse modules and add another verification with them.

==> cnnmodularity copy/motivationtb.tex <==
\begin{table}[htp]
	\footnotesize
	\centering
	\caption{Scenarios Created Based on Figure \ref{fig:overview}.}
	\label{tb:motivating}
\begin{tabular}{|l|c|c|}
	\hline
\textbf{Strategies}                                                                      & \textbf{Top-1 Acc}                  & \textbf{Top-5 Acc}                  \\
\hline
\hline
Initial Model                                                                   & 26.6\% &50.4\% \\
\hline
MA& 26.0\% & 50.4\% \\
\hline
Option 1                                                                        & 27.2\% & 54.6\% \\
\hline
Option 2                                                                        &                   25.0\%         &           50.4\%                 \\
\hline
Option 3                                                                        &            24.0\%                &   48.2\%  \\
\hline        
Option 4                                                                        &            25.3\%                &   50.8\%  \\
\hline                 
\end{tabular}
%\vspace{-10pt}
\end{table}

==> cnnmodularity copy/related.tex <==
\section{Related Works}
\label{sec:related}
There is a vast body of work~\cite{backus1957fortran, backus1960report, dijkstra2001go, dijkstra1970notes, dijkstra1982role, parnas1972criteria,  liskov1974programming, parnas1976design, america1990designing, dhara1997forcing, cardelli1997program, flatt1998units, tarr1999n} on software decomposition
that has greatly influenced us to decompose CNN model into reusable and replaceable modules.
% Here, we discuss the closest works carried in enabling the notion of decomposition in deep learning models.

The closest work is by Pan and Rajan~\cite{pan2020decomposing}, where the dense-based model has been decomposed into modules to enable reuse and replacement in various contexts. Though this work has motivated to decompose a CNN model into modules, the dense-based approach cannot be applied due to: 1) the shared weight and bias architecture in convolution layers, and 2) support for layers other than dense.
% , and 3) prior work suffers heavily on the inter-dataset reuse and replacement scenarios. 
Also, this work did not evaluate the impact of decomposition on $CO_2e$ emission during training. % Fix the 1, 2, 3

Ghazi~\etal~\cite{ghazi2019recursive} have introduced modular neural networks to incorporate memory into the model. They have proposed a hierarchical modular architecture to learn an output class and classes within that output class. Though this work has been able to increase the interpretability of the network by understanding how inputs are classified, the modules are not built to enable reusability or replaceability. Other works on modular networks~\cite{andreas2016neural, hu2017learning} have learned how different modules communicate with others to achieve better training. Also, capsule networks~\cite{hinton2000learning, sabour2017dynamic} can be utilized to incorporate memory into deep neural networks. In capsule networks, each capsule contains a set of features, and they are dynamically called to form a hierarchical structure to learn and identify objects. However, modules decomposed by our approach can be reused or replaced in various scenarios without re-training.

\citeauthor{sairam2018hsd}~\cite{sairam2018hsd} have proposed an approach to convert a CNN model into a hierarchical representation. At each level, nodes representing similar output classes are clustered together, and each cluster is decomposed further down the tree. Finally, with parameter transfer, the tree-based model is trained. While, in that work, a sub-section of the tree-based can be reused for a subset of the output classes, our approach decomposes a trained CNN model into reusable and replaceable modules to build a model for a new problem (intra and inter dataset) without retraining. Furthermore, we have shown that reusing and replacing modules decreases CO2e consumption significantly. 


==> cnnmodularity copy/results.tex <==
\section{Evaluation}
\label{sec:results}
\input{tbrq1.tex}
In this section, we discuss the experimental settings. Furthermore, we discuss the performance of decomposing the convolutional neural network into modules by answering three research questions, 1) does decomposition involve cost?, 2) how module reuse and replacement can be done compared to retraining a model from scratch?, and 3) does reusing and replacing the decomposed modules emit less $CO_2$?
\subsection{Experimental Settings} 
%Here, we discuss the type of the datasets, model, and computational metrics used,
\subsubsection{Datasets} We evaluate our proposed approach based on three widely used and well-vetted datasets.

\noindent\textbf{CIFAR-10 (C10)~\cite{krizhevsky2009learning}:} This dataset comprises of 3-D images of different objects. It has 10 output classes, and the dataset is divided into training and testing datasets. The training dataset has 50,000 images, and the testing dataset has 10,000 images.  
%The output classes are airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. Each of the images is of size (32, 32, 3), where the length, width, and color channels are 32, 32 pixels, and three dimensions, respectively.

\noindent\textbf{CIFAR-100 (C100)~\cite{krizhevsky2009learning}:} This dataset has 100 output classes. This is widely used to evaluate CNN-based studies due to the complexity of the dataset. Here, there are 50,000 training images and 10,000 testing images. The image size is similar to the CIFAR-10.

\noindent\textbf{ImageNet-200 (I200)~\cite{le2015tiny}:} This dataset is very popular and widely used to measure the scalability of CNN-based applications. Unlike the previous two datasets, the total number of output classes is 200. 
ImageNet dataset has been designed to help the computer-vision related task in machine learning. 
This dataset has 80,000+ nouns (name of the output class), and for each class, there are at least 500 images associated with it. This dataset has been used in training models in real-life scenarios. However, due to the complexity of the dataset, a smaller dataset with similar complexity has been made public for research purposes. This dataset (ImageNet-tiny) comprises 200 types of images. The training dataset has 100000 images, and the testing has 10000 images. 
%There are 3 different variations of the dataset, where the length and width of the images are 224, 64, and 32. In our experiments, we used the 64 version of the dataset to reduce the time-complexity of training such networks and have an experimental dataset that is different from CIFAR-10 and CIFAR-100 in terms of the image size.. 
\subsubsection{Models} We used the ResNet~\cite{he2016deep, he2016identity} models to evaluate our proposed approach. In a ResNet model, there are multiple blocks present and each block consists of \texttt{Convolution}, \texttt{Add}, and \texttt{Activation} layer. There are two versions of ResNet, the original version, where there is a stack of \texttt{Convolution}, \texttt{Add}, and \texttt{Batch Normalization} layers are put together to form a residual block, and those residual blocks build the network. In the second version, the residual block is modified to form a bottleneck layer with \texttt{Convolution}, \texttt{Add}, and \texttt{Batch Normalization}. We performed our evaluation against the first version of the network for simplicity and to reduce the training time and resources. Each such version can either have \texttt{Batch Normalization} layer or not as described in the original paper. Since \texttt{Batch Normalization} is only used to train and does not participate in the prediction, we chose the model without \texttt{Batch Normization} to reduce the training time as some of our experiments include training models multiple times. We used ResNet-20, ResNet-32, and ResNet-56, where 3, 5, and 9 residual blocks are present with 21, 33, and 57 convolution layers, respectively. The reported model accuracies are different from the original paper, as we trained the model from scratch with 200 epochs.
\subsubsection{Metrics Used}

\textbf{Accuracy.} We compute the composed accuracy of the decomposed modules as shown in the prior work~\cite{pan2020decomposing}. Pan~\etal computed the top-1 accuracy for all the experiments, whereas we compute both top-1 and top-5 accuracies. 
%In top-5 accuracy computation, each image is classified into 5 output classes and matched with labels provided with the dataset. 

\textbf{Jaccard Index.} Similar to the prior work, we compute the variability between the model and the modules using Jaccard Index.

%To observe the variability between the model and the decomposed modules, Jaccard Index has been computed, which is the same computation metric used by the prior work.

\textbf{$\boldsymbol{CO_2e}$ Emission.} In this context, we refer to $CO_2e$ as carbon dioxide and equivalent gases. These gases are harmful to humankind and the earth due to various reasons. One of them is that they are heat-trapping gases, and the excess presence of such gases can increase the average temperature of the earth, which can lead to several devastating circumstances. To measure the total emission of such gases due to computation, we utilize the metrics used by Strubell~\etal~\cite{strubell2019energy}. The total power consumption during the training is measured as ,
\begin{equation}
\label{eq:1}
p_t=\frac{1.58t(p_c+p_r+gp_g)}{1000}
\end{equation}
In this equation, $p_c$, $p_r$, $p_g$, and $g$ denote the average power consumption of CPU, DRAM, GPU, and the total number of GPU cores, respectively. The $t$ denotes the time. Here, 1.58 denotes the PUE co-efficient, which is the same value used in the prior work. We performed our experiment on iMac with 4.2 GHz Quad-Core Intel Core i7 and 32 GB 2400 MHz DDR4 RAM. Since we do not have any GPU, both $g$ and $p_g$ are zero. The power consumption has been measured using Intel Power Gadget
~\cite{intel}. %[Add at the End]
Finally, the $CO_2e$ emission has been computed as,
\begin{align}
CO_2e=0.954p_t
\end{align}

==> cnnmodularity copy/rq1.tex <==
\subsection{Results}
In this section, we evaluate our approach to understand the cost involved in decomposition, whether the decomposed modules can be reused or replaced, and how decomposition can be beneficial compared to training from scratch.
\subsubsection{Does Decomposing CNN Model into Module Involve Cost?}
\label{subsec:rq1}
%\input{tbrq1.tex}
\input{tbintrareuse1.tex}
\input{tbinterreuse1.tex}
To understand how decomposing CNN models into modules performs, we evaluate our approach on 9 datasets and model combinations. First, we decompose the CNN model into small modules, and then we compose them to evaluate how these composed modules perform compared to the trained CNN models. In Table \ref{tb:rq1}, the composed accuracy of the decomposed modules and the trained models' accuracy have been shown. We report the top-1 and top-5 accuracies of the models. Here, in the first and second columns, we show the top-1 and top-5 accuracy of the model. Whereas, in columns 3-11, the accuracy shown is from the composition of the decomposed modules. While composing the modules, we apply the voting-based approach that is similar to the prior work. Also, we compute the Jaccard index (JI) to identify the average variability between the modules and the model. Lesser value of the JI represents better decomposition as the modules are desired to be significantly different from the model. 
Suppose the value of the Jaccard index is very high. In that case, it denotes that the module has essentially become similar to the model.
While the lower JI is a criterion for better decomposition, the cost is another criteria to be considered while decomposing a model into modules. In this study, our objective is to have the least cost of decomposition with the most dissimilarities between the modules and the model.
%In top-5 accuracy, we identify five output classes based on the accuracy corresponding to each output class. While evaluating each proposed approach, we compute the top-1 and top-5 accuracy for the composition of the decomposed modules and compare that with the trained model's accuracy. 
%Furthermore, the Jaccard Index has been computed to understand the difference between the model and decomposed modules. While decomposing a model into modules, we have two goals, 1) reduce the cost of decomposition and 2) increasing the difference between the model and decomposed modules. For the latter, if the difference between the model and decomposed modules is very small, then decomposition is not entirely achieved, and the model and modules are the same.
%In this study, we first used our proposed concern identification approach with the concern channeling approach to convert $n$-classifier to a binary classifier. In order to overcome the challenges of the shared weights, we utilized a map-based technique. To reduce the computation and resources, we only store the co-ordinate of the nodes that do not participate in the decision of certain modules. While predicting, we convert the corresponding nodes into zeroes and continue the computation for the successive layers. We built a \textit{numpy} based prediction operation that takes the input, compute the sliding window, and compute the output for nodes that are not in the list of deactivated nodes using the shared weight and bias, but for the nodes that are in the list of deactivated nodes, we convert them into zeros and the output of that layer has been used as the input to the next layer and follow the model structure. 
We found that in all the cases, there is a cost involved while decomposing. For instance, our first approach identifies the concern, adds negative examples, and finally modularizes the concern involves 3.46\% and 2.54\%  (top-1 and top-5) of loss of accuracy with an average Jaccard index 0.50. Whereas applying dense-based backtracking, the loss has reduced. The average loss with this approach is 1.77\% and 0.85\%, and the average Jaccard index is 0.63. For approach involving the backtrack through the convolution layer includes a loss of 1.86\% and 1.93\% accuracy with an average 0.64 Jaccard index. For the further experiments, we choose the second approach as the loss is the least of all. Based on these results, we can conclude that decomposition is possible in CNN models. However, it involves a small cost, and the modules produced are significantly different from the models.
%From Table \ref{tb:rq1}, we found that the second approach (Dense-based backtracking) does the best in terms of accuracy and Jaccard index combination. Also, overall, we have a 2.38\% loss when top-1 accuracy has been computed, and for top-5 accuracy, we have a 0.81\% loss. The decomposed modules have an average 0.54 Jaccard index that indicates that the modules are significantly different from the models. 
%Furthermore, we compute the differences among the modules and found that, on average, the Jaccard index is A, which indicates that the modules are not similar to each other. While decomposing, this is a desirable quality as the modules created are different from each other, rather than creating a small sub-network that has the same structure for all the convolution layers and is only different in the output layer. 
For further studies, we used the dense-based backtracking technique.

==> cnnmodularity copy/rq2.tex <==
\subsubsection{How module reuse and replacement can be done compared to retraining a model from scratch?} Here, we evaluate how decomposed modules can be reused and replaced in various scenarios.
\label{subsec:rq2}
\input{tbintrareplace.tex}
\input{tbinterreplace.tex}

\textbf{Reusability:} Table \ref{tb:reuse}, and \ref{tb:interreuse} show two different reuse scenarios: 1) intra-dataset reuse, 2) inter-dataset reuse.

In intra-dataset reuse, we build a model by taking two output classes from a dataset and building a new model. For instance, output classes 0 and 1 have been taken from CIFAR-10, and we evaluate the accuracy by combining the decomposed modules for output classes 0 and 1 (we represent the output class with their index in the dataset). We compare the performance with retraining a model with the same structure with the same output classes and measure the accuracy. We took the best model for each dataset (based on the trained model accuracy) and the modules created from that. For CIFAR-10, CIFAR-100, and ImageNet-200, the best model in terms of training accuracy are ResNet-56, ResNet-20, and ResNet-20, respectively. Since these models take a long time to train, we performed the experiments for 4 output classes randomly chosen from the dataset to evaluate the reusability scenarios. In Table \ref{tb:reuse}, the intra-dataset reuse scenarios are reported. C1, C2, C3, and C4 denote the four randomly chosen classes, and they are different for each dataset.
%In the column, we have the name of the output class, e.g., \texttt{C10-Class1} denotes the first randomly chosen output class from CIFAR-10 dataset. We store the randomly chosen output class and train a model with the same set of output classes. In column \texttt{Module} and \texttt{Model}, the composed accuracy of the decomposed modules and the accuracy of the trained model has been denoted, respectively. 
Since we take 2 output classes in each experiment, the total number of choices for a dataset with $n$ output classes under experiment is $n \choose 2$. In our cases, we take 4 output classes from each dataset to evaluate, and the total choices would be $4 \choose 2$ or 6. For CIFAR-10, reusing the modules increase 6.6\% accuracy, on average. For CIFAR-100, there is an average 0.67\% loss, but 4/6 cases reusing the modules perform better than the trained model. For ImageNet, there is an average 1.5\% increase in accuracy. Overall, the gain in the accuracy in intra-dataset reuse is 2.5\%. 

In inter-dataset reuse, we take two output classes from different datasets and build a binary classification-based problem. For example, output classes 1 and 2 have been taken from the CIFAR-10 and CIFAR-100 datasets, respectively. We compute the accuracy the same way as we did for intra-dataset reuse scenario. Since the model structure of the decomposed modules for two datasets are different, e.g., the decomposed modules for CIFAR-10 follow the model structure of ResNet-56, whereas it is ResNet-20 for CIFAR-100. The best model in terms of accuracy has been taken for retraining. We did a pilot study and found that ResNet-20 does better in terms of accuracy for the inter-dataset reuse scenario for CIFAR-10 and CIFAR-100 datasets. To overcome overfitting, we store the checkpoints for all training-based evaluations and report the last checkpoint with the best validation accuracy. In Table \ref{tb:interreuse}, the inter-dataset reuse scenarios are reported. We found that inter-dataset reuse has a non-trivial cost. In this case, the loss of accuracy is 12.06\%. 
Our intuition is that since these modules originate from a different dataset, they still have some traits of the parent dataset. In fact, by applying the tangling identification approach, we deliberately add some non-concerned examples to distinguish between the concerned and the non-concerned examples. 
%However, when modules are reused or replaced in a scenario where the non-concerned output classes are different, these modules perform worse. 
To alleviate the effect, we perform a continuous learning-based approach, where we re-apply the tangling identification with the unseen output class(es). 
%We describe the approach in the following paragraph.
We found that enabling continuous learning can reduce the cost of decomposition significantly. The overall loss while reusing modules is 7.63\%, which is a 4.4\% gain compared to the previous reusability approach. Since the input size of the CIFAR-10 and CIFAR-100 images are not the same as ImageNet-200, both training a single model and reusing modules cannot be done. 
% This is similar to heterogeneous modules discussed by 
% Shaw~\etal~\cite{shaw1995abstractions}, where the input type of the two modules is different. 
% TODO: move to conclusion and future work 

\textbf{Replaceability:}
Similar to the reusability scenario, we evaluated both inter and intra-dataset reuses. For intra dataset reuse, we replace a module decomposed from a model with less accuracy with a module for the same output class decomposed from a model with higher accuracy. In Table \ref{tb:intrareplace}, we report the evaluation for replacing the module. For each dataset, we evaluate for 10 output classes to match the total number of classes for all the datasets. For CIFAR-10, we replace a module decomposed from ResNet-32 with a module for the same output class decomposed from ResNet-20. We found that the intra-dataset reuse increases the accuracy by 0.7\% and 1.0\% for top-1 and top-5 accuracy, respectively in comparison to the prior composed accuracy of the decomposed modules. In fact, 80.0\% (24/30) and 83.3\% (25/30) times replacing a module does the better or the same compared to the composed accuracy of the decomposed modules for top-1 and top-5 accuracy, respectively. Also, for 33.3\% and 66.7\% cases, reusing modules does better than the model accuracy for top-1 and top-5 accuracies, respectively.
Although we incorporated the continuous learning approach, there is no significant increase in accuracy  (top-1: 0.02\%  and top-5: 0.01\%).

Inter-dataset replacement scenarios are reported in Table \ref{tb:interreuse}. To reduce the experiment time, we replace a module from CIFAR-10 with a module taken randomly from CIFAR-100 and report both composed accuracy and the accuracy of the trained model for four different output classes. We found that for top-1 accuracy, there is a 2.5\% accuracy increase, and for top-5, there is a loss of 7.1\%, on average.
\input{motivationtb.tex}

\noindent\textbf{Motivating Example.} Here, we recreate the example shown in Figure \ref{fig:overview}. Since human face and Gorilla images are not present in the ImageNet-200 dataset, we added two classes from the ImageNet large dataset. However, there is no class specifically categorized as ``human face'' in the dataset. So, we take the closest class that contains the images of different persons.
First, we build a model with 202 (ImageNet-200 + Person + Gorilla) output classes. For the first option, we create a hypothetical model that does not exhibit faulty behavior. We do that by training a model with more epochs (+100 epochs) and achieve higher accuracy (+1.8\%). Then, we decompose the model into modules. Then, we replace the Gorilla module with the module created from the second model. In the second option, we train a model with Person and Gorilla examples and replace the faulty Gorilla module with the newly created one. In the third option, we remove the Gorilla module from the set of modules. Finally, in the fourth option, if the original model predicts Person or Gorilla, we re-verify with the modules created from the 2-class classification model in the second option. The evaluation has been shown in Table \ref{tb:motivating}, and we found that enabling the replacement and reuse of modules can solve the problem. Based on the need and available resources, users can pick any of the four options.

==> cnnmodularity copy/rq3.tex <==
\subsubsection{Does reusing and replacing the decomposed modules emit less $CO_2e$?}
\label{subsec:rq3}
\begin{figure}[!ht]
	\centering
	\includegraphics[, trim={2cm 7cm 0cm 7cm}, width=1.12\linewidth]{combined.pdf}
	\caption{Comparison of $CO_2e$ Emission.}
	\label{fig:c02}
	%	\vspace{-15pt}
\end{figure}
Strubell~\etal~\cite{strubell2019energy} have identified that training a model often emits six times more $CO_2e$ than a car emits over a year. To understand how decomposition can help to reduce the harmful effect, we measure the $CO_2e$ emission for both intra and inter-dataset reuse and replace scenarios. First, we start computing the power consumption before executing the program. Then, we measure the average power drawn by other tasks running in the background for 10 sec and compute the average power drawn by CPU and DRAM. We negate these two values to separate the resource consumption of the program and other background tasks. Then, we measure the power consumption for each 100 ms (default for Intel Power Gadget). 
Figure \ref{fig:c02} shows the $CO_2e$ emission for different scenarios. We do not show intra dataset replacement scenarios as that cannot be compared with training from scratch.
For training scenarios, we build the model from scratch, and after training, we predict the same set of images. This experimental setting has been done to compare a similar situation, where developers need to build and predict inputs. The value reported in the figure is the average $CO_2e$ consumption for all the experimented scenarios described in \S\ref{subsec:rq2}. Also, since the epoch has been fixed for each retraining, the power consumption is somewhat fixed for each retraining scenario. However, the best model can be found earlier. For instance, a model is trained with 100 epochs, but the best model is found at the 20th epoch. To remove the effect of overfitting, we compute the power consumed until the return of the best model and report that in the figure. 
We found that for reuse scenarios, decomposition reduces the $CO_2e$ consumption by 
23.7x and 18.3x for the fixed epoch and the best model scenarios, respectively. For replacement scenarios, it is 42x and 31.5x, respectively. If we apply the continuous learning-based approach, there is a slight increase in resource consumption, but still significantly less than training from scratch. Also, we computed the additional $CO_2e$ consumption for the one-time decomposition approach and found that on average 116, 371, and 3800 lbs of $CO_2e$ has been generated for decomposing CIFAR-10, CIFAR-100, and ImageNet-200 models, respectively. The overhead is significantly lower for CIFAR-10 and CIFAR-100 compared to training a new model for both reuse and replace scenarios. However, for ImageNet-200, the overhead is high, but it is a one-time operation that can enable both reuses and replacements at a very low cost.



%We found that reusing the decomposed modules and predicting the test images can reduce the $CO_2$ emission by $\sim$22x and $\sim$19x for CIFAR-10 if we consider the power consumed when the retraining is done with fixed epoch and retraining till the best model is found, respectively. Also, the overall power consumption for the CIFAR-10 scenario is more than in other cases. Here, we used the best model from each dataset based on the training accuracy. For CIFAR-10, the best model is ResNet-56, which is the most complex model in our experimental models, whereas for CIFAR-100, the chosen model is ResNet-20, and it is the same for ImageNet-200. Due to increased complexity and the parameters for the ResNet-56 model, the resource consumption for retraining the model and reusing the decomposed modules is more than any other scenario. Similarly, for CIFAR-100 intra dataset reuse, the reduction of $CO_2$ is $\sim$53x and $\sim$33x. For ImageNet-200, it is $\sim$58x and $\sim$47x. For inter dataset reuse, we have two approaches, one with continuous learning and one without that. Without applying the continuous learning, the $CO_2$ emission has been reduced by $\sim$12x and $\sim$10x for two previously mentioned scenarios. Whereas, if we apply the continuous learning process, the reduction of $CO_2$ is $\sim$5x and $\sim$4x. On average, the $CO_2$ emission can be reduced $\sim$44x and $\sim$33x for intra dataset reuse based on the fixed epoch or variable epoch-based approach. Given the size, complexity, and wide usage of the CNN models, reducing $CO_2$ emission can help us restore the harm done to our planet. With the tremendous increase in computational power in today's world, resource consumption has often been neglected when it comes to increasing performance; however, while building/rebuilding models, both performance and resource consumption should be considered.

==> cnnmodularity copy/tbMotiv.tex <==
%\begin{table*}[]
%	\footnotesize
%	\centering
%	\caption{Detailed Steps, Pros, and Cons of Different Approaches using Decomposed Modules.}
%	\label{tb:motiv}
\begin{tabular}{|p{1cm}|p{8.5cm}|p{2.8cm}|p{3.8cm}|}
	\hline
\multicolumn{1}{|c}{\textbf{Strategies}}                                                                      & \multicolumn{1}{|c|}{\textbf{Description}}                  & \multicolumn{1}{c}{\textbf{Pros}}          & \multicolumn{1}{|c|}{\textbf{Cons}}        \\
\hline
\hline
\multirow{1}{*}[-2.8em]{\textbf{Option 1}}                                                                        & We decompose the faulty CNN model into modules for each output class. Each such module is a binary classifier that classifies whether an input belongs to the output class (for which the module is decomposed) or not. Now, suppose we have another working model trained with the same or a subset of the dataset with the gorilla and person output labels. This new model does not exhibit the behavior present in the faulty one. Then, we can replace the faulty gorilla module with the working gorilla module.& Since the module belong to the same dataset as the faulty model, the module will have sufficient information to both recognize and distinguish new inputs. & These models are massive, and training is very sufficiently costly. Thus, the availability of a similar trained model with the Gorilla class may not be feasible for all conditions. \\
\hline
\multirow{1}{*}[-2.61em]{\textbf{Option 2}}                                                                    &                             We decompose the faulty model into modules. Moreover, we train a new model with a person and gorilla classes and validate that the trained model does not demonstrate faulty behavior. We decompose the newly trained model into two modules (gorilla and person) and replace the faulty gorilla module with the new decomposed gorilla module.  &     Training with a small dataset requires less resources in comparison to training the whole dataset.       & Decomposition can not alone solve the problem. However, the decomposition bundled with the traditional training could help in this situation.  \\
\hline
\multirow{1}{*}[-.61em]{\textbf{Option 3}}                                                                   &            We decompose the faulty model into modules and remove the gorilla module from the collection. In this scenario, there is no cost of retraining involved.              &    This method is cost-effective.  & The actual problem of faulty classification has not been addressed.\\
\hline        
\multirow{1}{*}[-1.61em]{\textbf{Option 4}}                                                                         &            We can also reuse the person and gorilla module from a working model without the faulty behavior. If any input is classified as a person or gorilla using the faulty model, we reuse the working modules to verify it further.           &   This approach is cost effective and used for further verification. & Since this approach involves another layer of verification using modules, there is an overhead present. \\
\hline                 
\end{tabular}
%\end{table*}

==> cnnmodularity copy/tbinterreplace.tex <==
\begin{table*}[]
	\caption{Intra Dataset Replace.}
	\footnotesize
	\centering
	\label{tb:intrareplace}
	\vspace{-10pt}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
		\multicolumn{13}{c}{\textbf{Top-1 Accuracy}}\\
		\hline
		\textbf{Dataset} & \textbf{TMA} & \textbf{Prior MA} &\textbf{RM0} & \textbf{RM1} &\textbf{RM2} & \textbf{RM3} & \textbf{RM4} & \textbf{RM5} & \textbf{RM6} & \textbf{RM7} & \textbf{RM8} & \textbf{RM9} \\
		\hline
		\hline
		\textbf{CIFAR-10} & 85.3\% & 78.6\% & 80.6\% & 79.2\% & 80.0\% & 80.9\% & 80.7\% & 80.2\% & 79.8\% & 79.6\%& 79.4\%& 79.6\% \\
		\hline
		\textbf{CIFAR-100} & 44.5\% & 41.2\% & 40.7\% & 41.0\% & 41.2\%& 41.1\% & 41.2\% & 41.1\% & 41.2\% & 41.2\% & 41.1\% & 41.0\% \\
		\hline
		\textbf{ImageNet-200} & 31.8\% & 31.5\% & \textbf{ 32.4\% }   &    \textbf{ 32.2\%}&       \textbf{32.3\%}&       \textbf{32.0\%}&       \textbf{32.3\%}&       \textbf{32.4\%}&       \textbf{32.4\%}&      \textbf{33.3\%}&       \textbf{33.2\%}&  \textbf{33.3\%}\\
		\hline
		\multicolumn{13}{c}{\textbf{Top-5 Accuracy}}\\
		\hline
		\textbf{Dataset} & \textbf{TMA} & \textbf{Prior MA} &\textbf{RM0} & \textbf{RM1} &\textbf{RM2} & \textbf{RM3} & \textbf{RM4} & \textbf{RM5} & \textbf{RM6} & \textbf{RM7} & \textbf{RM8} & \textbf{RM9} \\
		\hline
		\hline
		\textbf{CIFAR-10} & 99.2\% & 98.1\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\% }\\
		\hline
		\textbf{CIFAR-100} & 74.6\% & 71.0\% & 70.7\% & 70.8\% & 71.0\% & 70.9\% & 71.0\% & 71.0\% & 71.1\% & 71.1\% & 70.9\% & 70.9\% \\
		\hline
		\textbf{ImageNet-200} & 58.6\% & 58.0\% &  \textbf{59.3\%}     & \textbf{59.1\%}  &       \textbf{59.1\%}&       \textbf{59.2\%}&       \textbf{59.0\%}&       \textbf{59.2\%}&       \textbf{59.1\%}&     \textbf{59.2\%}  &      \textbf{59.2\%}&\textbf{59.1\%}\\
		\hline
	\end{tabular}%
	
	TMA: Trained Model Accuracy, MA: Composed Module Accuracy, RM\{x\}: Replace Module x with another Module for x.
\end{table*}
\begin{table*}[]
	\caption{Inter Dataset Replace. (All results are in \%.)}
	\footnotesize
	\centering
     \begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
     	\hline
    \multirow{2}{*}{\backslashbox{\textbf{C100}}{\textbf{C10}}}& \multicolumn{4}{c|}{\textbf{C1}}         & \multicolumn{4}{c|}{\textbf{C2}}         & \multicolumn{4}{c|}{\textbf{C3}}         & \multicolumn{4}{c|}{\textbf{C4}} \\
    	\cline{2-17}
    	& \textbf{M1} & \textbf{D1} & \textbf{M5} & \textbf{D5} & \textbf{M1} & \textbf{D1} & \textbf{M5} & \textbf{D5} & \textbf{M1} & \textbf{D1} & \textbf{M5} & \textbf{D5} & \textbf{M1} & \textbf{D1} & \textbf{M5} & \textbf{D5} \\
    	\hline
    	\hline
    	\textbf{C1}     & 86.2\ & \textbf{87.3}\ & 99.6\ & 95.9\ & 83.1\ & \textbf{87.4}\ & 98.9\ & 95.6\ & 86.1\ & \textbf{87.1}\ & 99.5\ & 95.4\ & 86.7\ & \textbf{87.0}\ & 99.6\ & 95.4\ \\
    	\hline
    	\textbf{C2}     & 85.3\ & \textbf{86.3}\ & 99.2\ & 90.8\ & 82.7\ & \textbf{86.3}\ & 98.9\ & 90.5\ & 84.6\ & \textbf{86.1}\ & 99.1\ & 90.3\ & 87.6\ & 86.0\ & 99.4\ & 90.3\ \\
    	\hline
    	\textbf{C3}     & 86.2\ & \textbf{88.1}\ & 99.4\ & 91.5\ & 81.8\ & \textbf{88.3}\ & 98.8\ & 91.3\ & 86.2\ & \textbf{88.0}\ & 99.0\ & 91.2\ & 87.9\ & 87.8\ & 99.6\ & 91.3\ \\
    	\hline
    	\textbf{C4}     & 84.7\ & \textbf{89.9}\ & 99.2\ & 91.4\ & 82.6\ &\textbf{89.7}\ & 98.7\ & 91.1\ & 85.0\ & \textbf{89.5}\ & 98.8\ & 91.1\ & 86.6\ & \textbf{89.3}\ & 99.4\ & 91.1\ \\
    	\hline
    \end{tabular}

M1 and  M5: Top-1 and Top-5 Accuracy for Trained Model D1 and D5: Top-1 and Top-5 Composed Accuracy for Decomposed Modules.
\end{table*}





==> cnnmodularity copy/tbinterreuse1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htp]
	\caption{Inter Dataset Reuse.}
	\centering
	\footnotesize
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}
	\hline
	\multirow{2}{*}{\backslashbox{\textbf{C100}}{\textbf{C10}}}& \multicolumn{3}{c|}{\textbf{C1}} & \multicolumn{3}{c|}{\textbf{C2}} & \multicolumn{3}{c|}{\textbf{C3}} & \multicolumn{3}{c|}{\textbf{C4}} \\
	\cline{2-13}
	& \multicolumn{1}{|l}{\textbf{TMA}} & \multicolumn{1}{l|}{\textbf{MA}} & \multicolumn{1}{l|}{\textbf{MMA}} & \multicolumn{1}{l|}{\textbf{TMA}} & \multicolumn{1}{l|}{\textbf{MA}} & \multicolumn{1}{l|}{\textbf{MMA}} & \multicolumn{1}{l|}{\textbf{TMA}} & \multicolumn{1}{l|}{\textbf{MA}} & \multicolumn{1}{l|}{\textbf{MMA}} & \multicolumn{1}{l|}{\textbf{TMA}} & \multicolumn{1}{l|}{\textbf{MA}} & \multicolumn{1}{l|}{\textbf{MMA}} \\
	\hline
	\hline
	\textbf{C1} & 97.8\% & 83.0\% & 91.5\% & 96.7\% & 87.9\% & 92.1\% & 96.6\% & 86.0\% & 91.5\% & 98.8\% & 87.2\% & 93.8\% \\
	\hline
	\textbf{C2} & 95.5\% & 82.4\% & 89.2\% & 98.6\% & 87.5\% & 88.1\% & 95.6\% & 85.2\% & 89.9\% & 99.7\% & 84.1\% & 89.0\% \\
	\hline
	\textbf{C3} & 98.4\% & 78.2\% & 87.5\% & 97.9\% & 79.5\% & 88.5\% & 94.6\% & 80.2\% & 89.2\% & 99.6\% & 81.6\% & 87.9\% \\
	\hline
	\textbf{C4} & 98.0\% & 88.3\% & 88.1\% & 97.2\% & 88.6\% & 88.1\% & 94.7\% & 86.7\% & 90.3\% & 99.0\% & 88.9\% & 91.9\% \\
	\hline
\end{tabular}\\
TMA: Trained Model Accuracy, MA: Composed Module Accuracy, and MMA: Modified Module Accuracy.
\label{tb:interreuse}
\end{table*}

==> cnnmodularity copy/tbintrareplace.tex <==
%\begin{table*}[]
%	\caption{Intra Dataset Replace.}
%	\footnotesize
%	\centering
%	\label{tb:intrareplace}
%	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
%		
%		\multicolumn{13}{c}{Top-1 Accuracy}\\
%		\hline
%		\textbf{Dataset} & \textbf{TMA} & \textbf{Prior MA} &\textbf{RM0} & \textbf{RM1} &\textbf{RM2} & \textbf{RM3} & \textbf{RM4} & \textbf{RM5} & \textbf{RM6} & \textbf{RM7} & \textbf{RM8} & \textbf{RM9} \\
%		\hline
%		\hline
%		\textbf{CIFAR-10} & 86.3\% & 79.5\% & \textbf{80.7\%} & \textbf{80.4\%} & \textbf{81.1\% }& \textbf{82.6\%} & \textbf{81.7\%} & \textbf{81.8\%} & \textbf{81.2\%} & \textbf{80.8\%} & \textbf{79.9\%} & \textbf{81.0\% }\\
%		\hline
%		\textbf{CIFAR-100} & 47.8\% & 42.7\% & 42.3\% & 42.5\% & \textbf{42.7\%} & 42.5\% & 42.6\% & \textbf{43.0\%} & 42.2\% & 42.6\% & \textbf{42.7\%} & 42.5\% \\
%		\hline
%		\textbf{ImageNet-200} & 31.2\% & 29.4\% &  \textbf{31.2\% }    &     \textbf{30.6\% } &       \textbf{31.0\%}&       \textbf{30.6\%}&       \textbf{30.8\%}&       \textbf{31.4\%}&       \textbf{31.6\%}&      \textbf{31.4\%} &       \textbf{31.4\%}&  \textbf{31.2\%}\\
%		\hline
%		\multicolumn{13}{c}{Top-5 Accuracy}\\
%		\hline
%		\textbf{Dataset} & \textbf{TMA} & \textbf{Prior MA} &\textbf{RM0} & \textbf{RM1} &\textbf{RM2} & \textbf{RM3} & \textbf{RM4} & \textbf{RM5} & \textbf{RM6} & \textbf{RM7} & \textbf{RM8} & \textbf{RM9} \\
%		\hline
%		\hline
%		\textbf{CIFAR-10} & 99.5\% & 98.2\% & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\% }\\
%		\hline
%		\textbf{CIFAR-100} & 73.8\% & 72.4\% & 71.1\% & 71.0\% & 71.3\% & 71.4\% & 71.3\% & 71.6\% & 71.5\% & 71.5\% & 71.1\% & 71.5\% \\
%		\hline
%		\textbf{ImageNet-200} & 55.2\% & 55.6\% &  \textbf{57.6\% }    & \textbf{ 57.4\%   }  &       \textbf{57.2\%}&       \textbf{57.2\%}&       \textbf{56.8\%}&       \textbf{57.4\%}&       \textbf{57.4\%}&     \textbf{57.2\% } &       \textbf{57.4\%}& \textbf{56.6\%} \\
%		\hline
%	\end{tabular}%
%
%TMA: Trained Model Accuracy, MA: Composed Module Accuracy, RM\{x\}: Replace Module x with another Module for x.
%\end{table*}

%\begin{table*}[]
%	\caption{Intra Dataset Reuse (Top-5 Accuracy)}
%	\small
%	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		
%	\end{tabular}%
%\end{table*}

==> cnnmodularity copy/tbintrareuse1.tex <==
\begin{table*}%
	\centering
	\footnotesize
		\caption{Intra Dataset Reuse. MA: Composed Module Accuracy, TMA: Trained Model Accuracy, C10: CIFAR-10, C100: CIFAR-100, I200: ImageNet-200, and C\{x\}: Output Label x}%
	%\begin{adjustbox}{width=\linewidth,center}
	\subfloat[CIFAR-10 and CIFAR-100 Reuse. \colorbox{moccasin}{Yellow} and \colorbox{magicmint}{Green} represent the CIFAR-10 and CIFAR-100 reuse scenarios, respectively.]{
		
			\begin{tabular}{|c|c|c|c|c|c|c|c|}
				\hline
				\multicolumn{2}{|c|}{\textbf{C10}}           & \multicolumn{2}{c|}{\textbf{C2}}                         & \multicolumn{2}{c|}{\textbf{C3}}                         & \multicolumn{2}{c|}{\textbf{C4}}                         \\ \hline
				\textbf{C100} & \textbf{C10}    & \textbf{TMA}                 & \textbf{MA}                  & \textbf{TMA}                 & \textbf{MA}                  & \textbf{TMA}                 & \textbf{MA}                  \\ \hline
				\hline
				\textbf{C1} & \textbf{C1} & \cellcolor[HTML]{FAEBD7}95.4\% &  \cellcolor[HTML]{FAEBD7}\textbf{98.8\%} &
				 \cellcolor[HTML]{FAEBD7}\textbf{84.7\%}  &
				  \cellcolor[HTML]{FAEBD7}\textbf{91.4\%} &  \cellcolor[HTML]{FAEBD7}\textbf{91.9\%} &
				  \cellcolor[HTML]{FAEBD7}\textbf{96.6\%}  \\ \hline
				\textbf{C2} & \textbf{C2} & \cellcolor[HTML]{AAF0D1}\textbf{91.0\%} & \cellcolor[HTML]{AAF0D1}\textbf{91.0\%} & 
				 \cellcolor[HTML]{FAEBD7}\textbf{93.2\%} &
				 \cellcolor[HTML]{FAEBD7}\textbf{99.3\%} &  \cellcolor[HTML]{FAEBD7}\textbf{92.2\%} &
				 \cellcolor[HTML]{FAEBD7}\textbf{99.3\%} \\ \hline
				\textbf{C3} & \textbf{C3} & \cellcolor[HTML]{AAF0D1}\textbf{96.0\%} & \cellcolor[HTML]{AAF0D1}\textbf{96.0\%} & \cellcolor[HTML]{AAF0D1}\textbf{95.0\%} & \cellcolor[HTML]{AAF0D1}\textbf{98.0\%} & \cellcolor[HTML]{FAEBD7}\textbf{81.2\%} & \cellcolor[HTML]{FAEBD7}\textbf{92.9\%} \\ \hline
				\textbf{C4} & \textbf{C4} & \cellcolor[HTML]{AAF0D1}100\% & \cellcolor[HTML]{AAF0D1}95.5\%   & \cellcolor[HTML]{AAF0D1}100\% & \cellcolor[HTML]{AAF0D1}96\%   & \cellcolor[HTML]{AAF0D1}\textbf{98.5\%}   & \cellcolor[HTML]{AAF0D1}\textbf{100\%} \\ \hline
				\multicolumn{2}{|c|}{\textbf{C100}}          & \multicolumn{2}{c|}{\textbf{C100-C1}}                        & \multicolumn{2}{c|}{\textbf{C100-C2}}                        & \multicolumn{2}{c|}{\textbf{C100-C3}}                        \\ \hline
			\end{tabular}
	}%
	\subfloat[ImageNet-200 Reuse.  \colorbox{moccasin}{Yellow} represents the ImageNet-200 reuse scenarios. \colorbox{black}{\textcolor{white}{Black}} represents the wrong combination of reuses.]{
		
			\begin{tabular}{|c|c|c|c|c|c|c|}
				\hline
				\multirow{2}{*}{\textbf{I200}}
				& \multicolumn{2}{c|}{\textbf{C2}}                        & \multicolumn{2}{c|}{\textbf{C3}}                      & \multicolumn{2}{c|}{\textbf{C4}}                                                        \\ \cline{2-7}
				& \textbf{TMA}                 & \textbf{MA}                  & \textbf{TMA}                & \textbf{MA}                 & \textbf{TMA}                                 & \textbf{MA}                                  \\ \hline
				\textbf{C1}           & \cellcolor[HTML]{FAEBD7}\textbf{90.00\%} & \cellcolor[HTML]{FAEBD7}\textbf{98.00\%} & \cellcolor[HTML]{FAEBD7}\textbf{93.0\%} & \cellcolor[HTML]{FAEBD7}\textbf{94.0\%} & \cellcolor[HTML]{FAEBD7}\textbf{92.0\% }                 & \cellcolor[HTML]{FAEBD7}\textbf{94.0\%}                \\ \hline
				\textbf{C2}           & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{FAEBD7}95.0\% & \cellcolor[HTML]{FAEBD7}88.0\% & \cellcolor[HTML]{FAEBD7}\textbf{95.0\% }                 & \cellcolor[HTML]{FAEBD7}\textbf{95.0\%}                  \\ \hline
				\textbf{C3}           & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{000000}       & \cellcolor[HTML]{000000}       & \cellcolor[HTML]{FAEBD7}\textbf{89.0\%}                  & \cellcolor[HTML]{FAEBD7}\textbf{94.0\% }                 \\ \hline
				\textbf{C4}           & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{000000}        & \cellcolor[HTML]{000000}       & \cellcolor[HTML]{000000}       & \cellcolor[HTML]{000000}{\color[HTML]{333333} } & \cellcolor[HTML]{000000}{\color[HTML]{333333} } \\ \hline
			\end{tabular}
	}
%\end{adjustbox}

	\label{tb:reuse}%
\end{table*}

%\begin{table}[]
%	\caption{Intra Dataset Reuse}
%	\footnotesize
%	
%	\label{tb:intrac10c100}
%\end{table}
%
%\begin{table}[]
%	\caption{Intra Dataset Reuse}
%	\footnotesize
%	\centering
%
%	\label{tb:intrai200}
%\end{table}

==> cnnmodularity copy/tbrq1.tex <==
\begin{table*}[htp]
	\centering
	\caption{Decomposition Effectiveness and the Variability between the Decomposed Modules and the Trained Model.}
\footnotesize
\label{tb:rq1}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{}                        & \multicolumn{2}{c|}{\textbf{Acc}} & \multicolumn{3}{c|}{\textbf{CI+TI+MC}} & \multicolumn{3}{c|}{\textbf{CI+TI+MC-BLN}} & \multicolumn{3}{c|}{\textbf{CI+TI+MC-BLN+MC-BI}} 
\\ 
\cline{2-12} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{Top 1}              & \textbf{Top 5}              & \textbf{Top 1}      & \textbf{Top 5}      & \textbf{JI}     & \textbf{Top 1}        & \textbf{Top 5}        & \textbf{JI}        & \textbf{Top 1}        & \textbf{Top 5}        & \textbf{JI}        \\ \hline
\hline
\textbf{CIFAR10-R20}                                                  & 87.1\%                        & 99.5\%                           & 86.9\%                & 96.0\%                   & 0.75            & 87.0\%                  & 99.4\%                     & 0.75               & 86.8\%                  & 95.8\%                     & 0.75               \\ \hline
\textbf{CIFAR10-R32}                                                  & 85.3\%                        & 99.2\%                           & 78.4\%              & 96.0\%                   & 0.51            & 78.6\%                  & 98.1\%                     & 0.51               & 78.4\%                  & 97.0\%                     & 0.51               \\ \hline
\textbf{CIFAR10-R56}                                                  & 86.7\%                        & 99.4\%                           & 84.0\%                & 93.9\%                   & 0.41            & 84.5\%                  & 98.9\%                     & 0.41               & 84.0\%                  & 93.9\%                    & 0.41               \\ \hline
\textbf{CIFAR100-R20}                                                 & 46.3\%                        & 75.2\%                        & 45.6\%                & 75.4\%                & 0.63            & 45.6\%                  & 75.4\%                  & 0.63               & 45.6\%                  & 75.4\%                  & 0.63               \\ \hline
\textbf{CIFAR100-R32}                                                 & 44.5\%                      & 74.6\%                        & 41.2\%              & 71.0\%                & 0.52            & 41.2\%                  & 71.0\%                  & 0.52               & 41.2\%                  & 71.0\%                  & 0.52               \\ \hline
\textbf{CIFAR100-R56}                                                 & 45.7\%                        & 75.1\%                        & 44.9\%                & 74.5\%                & 0.68            & 44.9\%                & 74.5\%                  & 0.68               & 44.9\%                  & 74.5\%                  & 0.69               \\ \hline
\textbf{ImageNet200-R20}                                              & 33.2\%                        & 59.7\%                      & 29.6\%                & 56.1\%              & 0.43            & 32.6\%                  & 59.7\%                & 0.75               & 32.6\%                  & 59.7\%                & 0.75               \\ \hline
\textbf{ImageNet200-R32}                                              & 31.8\%                        & 58.6\%                      & 21.0\%                & 58.0\%              & 0.33            & 31.5\%                  & 58.0\%                & 0.72               & 31.5\%                  & 58.0\%                & 0.72               \\ \hline
\textbf{ImageNet200-R56}                                              & 32.1\%                        & 58.7\%                      & 30.0\%                & 56.7\%              & 0.30            & 31.0\%                  & 57.8\%                & 0.71               & 31.0\%                  & 57.8\%                & 0.71               \\ \hline
\end{tabular}

Acc: Accuracy, CI: Concern Identification, TI: Tangling Identification, MC: Modularizing Concern, MC-BLN: Modularizing Concern: Backtrack to Last Convolutional Layer, MC-BI: Modularizing Concern: Backtrack to Input, and JI: Jaccard Index.
\end{table*}

==> cnnmodularity copy/technique1.tex <==
\subsection{Concern Identification}
%% I recommend edit this subsection to its readability
Concern Identification (CI) involves identifying the section of the CNN model, responsible for the single output class. As a result of this process, we remove nodes and edges in the model. In traditional CNN models for image classification, both convolution, and dense layers have the notion of node and edges, and we discuss the concern identification approaches for both the layers. %Compared to the prior work on decomposition, we identify the inactive output nodes at each layer.

\noindent\textbf{Dense Layers:}
%Here, we identify the \textit{concerned} section by updating or removing the edges connected to the nodes. 
Here, the concerned section can be identified by updating or removing the edges connected to the nodes. In a dense-based network, there is a one-to-one relationship between the edges connecting the nodes from different layers (including the bias nodes). For each edge, the originating and the incident nodes are unique except for bias, where the incident node is unique. The edges between nodes are removed or updated based on the value associated with the nodes. In this process, we identify nodes based on the assumption that ReLU has been used as the activation function. Since our work is focused on image-based classification models, ReLU is the most commonly used activation function for the hidden layers. Also, prior work on decomposition~\cite{pan2020decomposing} has been carried out with the same assumption.
%In fact, all the models available in Keras library for image classification have used ReLU as the activation function for the hidden layers~\cite{keras}.
%Furthermore, all the models available in the Keras library for image classification use ReLU as the activation function for the hidden layers~\cite{keras}.

First, we compute the value associated with the nodes by applying training inputs from the concerned output class. For an input, if the computed value at a node is $\le$0, then we remove all the incident and originated edges. We do that for all the concerned inputs from the training dataset. If the value associated with a node is $>$0 for some input and $\le$0 for other inputs, we do not remove that node. 
%However, edges that originated from the dense layer preceding the logit layer will have inactive nodes, and all the edges that originated from them will be removed, too. 
For instance, for a layer $L_d$, there are $n_{L_d}$ number of nodes, and the preceding and the following layer has $n_{L_{d-1}}$ and $n_{L_{d+1}}$ nodes, respectively. For any node at the layer $L_d$, there will be $n_{L_{d-1}}$incident edges and $n_{L_{d+1}}$ outgoing edges. Based on our computation, if a node $n_i$ is inactive (value $\le$0), then all the incoming and outgoing weight edges ($n_{i(L_{d-1})}$ + $n_{i(L_{d+1})}$) and one bias edge incident to $n_i$ will be removed. We do the same for all the hidden dense layers. 
\input{algoci.tex}

\noindent\textbf{Convolution Layers:}
%While dense layers have a one-to-one relationship between the nodes and edges, in the convolution layer, each weight is shared by all the nodes in the input and the output. 
In a convolutional layer, we identify the inactive sections in the output nodes by using a mapping-based technique that stores the position of the nodes that are not part of a module. 
In Algo.\ref{algo:concern}, we describe the steps involved in building
the map and storing the nodes' positions. First, we store the
weight and bias for all the layers. Then, we identify the parts of the
convolution layer that are not used for a single output class. 
%In a typical convolutional neural network for the image classification task, these two layers are associated with the weight and bias and take part in the learning process.
We start by computing all possible combinations of sliding windows at line \ref{algo1:10}. To build the sliding windows, we use the $stride$, $padding$ as input. Below, we describe each such parameter.


\textbf{Sliding Window.} In convolutional layers, instead of one input node at a time, a set of nodes are taken as an input for computation. For instance, in Figure \ref{fig:cnn}, the blue box is a sliding window. For each sliding window, one or more output nodes are created based on the size of the shared weight in the layer.

\textbf{Padding.} Two variations of padding is possible in CNN, zero-padding and with-padding. In zero-padding, the input is not changed. For with-padding, the input is padded based on the size of the sliding window, and the size of the output will be the same as the input. For the example shown in Figure \ref{fig:cnn}, we used the with-padding, and that adds padding with value zero and transforms the input into (5, 5, 3) size (the white boxes are the added padding).

\textbf{Stride.} This parameter controls the movement of the sliding window while computing the output. Stride along with the padding decides the output of the layer.

Once we compute the sliding windows (line \ref{algo1:10}), we feed inputs from the training dataset to our approach and observe the output value of that particular convolution layer. At line \ref{algo1:11}, we compute the output of the convolution layer based on S*W + B, where S, W, and B denote the sliding window, shared weight, and bias, respectively. Then, we monitor the value at each node (line \ref{algo1:12}-\ref{algo1:25}). If a node has a value $\le0$, we store the position of the node in our map. We initialize the map with all the nodes (for the first input) that have value $\le0$ (line \ref{algo1:14}-\ref{algo1:16}). The \textit{first} flag is used to denote this first input to the module. Then, we remove the nodes that are previously in the mapping list, but the nodes have a positive value for the input under observation (line \ref{algo1:17}-\ref{algo1:24}). We perform such operations to identify the section of the layer that is inactive for a particular concern.
For the batch normalization layer, there is no weight or bias involved, and the layer is utilized for normalizing the input based on the values learned during the training session. Max pooling and average pooling are utilized for reducing the size of the network using the pool size. For merge or add layer, we add the value computed from the two layers connected with this layer.

==> cnnmodularity copy/technique3.tex <==
\subsection{Tangling Identification}
%% I recommend edit this subsection to its readability
In concern identification, a module is created based on identifying the nodes and edges for a single output class. Since all the nodes and edges related to the other output classes in the dataset have been removed, the module essentially characterizes any input as the concerned output class or behaves as a single-class classifier. To add the notion of unconcerned output classes and able to distinguish between the concerned and unconcerned output classes, we bring back some of the nodes and edges to the module. In Tangling Identification (TI), a limited set of inputs belonging to the unconcerned output classes have been added. Based on the prior work, we add concerned and unconcerned inputs with a 1:1 ratio. For instance, if we have a problem with 200 output classes and build a module based on observing 1000 inputs from the concerned class, then we observe 5 inputs from each unconcerned class (5x199=995$\approx$1000).
\subsection{Modularizing Concerns}
\label{subsec:cm}

So far, we identify the section of the network that is responsible for an output class and added examples from unconcerned output classes. However, the module is still an $n$-class classification problem. We channel the output layer for each module to convert that into a binary classification-based problem. 
%Until now, the module created is a $n$-class classifier, where $n$ is the total number of output classes in the dataset. 
%Here, we modularize the concern and channel the output labels to convert the $n$-classification into a binary classification problem.
 However, before applying the channeling technique, we remove irrelevant nodes (do not participate in the classification task for a module) using a bottom-up backtracking approach. 
 %Our approach also supports other layers, e.g., pooling, merge/add.

\noindent\textbf{Dense Layers:}
We channel the out edges as described by the prior work~\cite{pan2020decomposing}. Instead of having $n$ nodes at the output layer ($L_{d}$, where $d$ is the total number of dense-based layers), two nodes (concerned and unconcerned output nodes) have been kept. For instance, the concerned output class for a module is the first output class in the dataset. We have $n$ output classes and $n$ nodes ($V_1, V_2, \dots, V_n$) at the output layer. Also, the layer preceding the output layer ($L_{d-1}$) has $n_{L_{d-1}}$ nodes. For each node at the output layer, there will be $n_{L_{d-1}}$ incident edges. For instance, the incoming edges for $V_1$ node will be $E_{11}, E_{21}, \dots, E_{n_{L_{d-1}}1}$, where $E_{n_{L_{d-1}}*1}$ (in this case, n=1) denotes that an edge is connected with $n_{L_{d-1}}^{th}$ node from $L_{d-1}$ layer and the first node at the output layer. For the module responsible for identifying the first output label, the edges incident to the first node (as the concerned node is $V_1$) at the output layer have been kept intact. However, all the other edges are modified. All the edges incident to any of the unconcerned nodes ($V_2$, $V_3$, $\dots$, $V_n$) at the $L_d$ layer will be updated by a single edge. The assigned weight for the updated edge is the mean of all the edges (same for bias). Then, that updated edge has been connected to a node at the output layer, which is the unconcerned node for the module. For a module, there will be two nodes at the output layer, $V_c$ and $V_{uc}$, where $V_c$ and $V_{uc}$ denote the concerned node and the unconcerned node. All the updated edges will be connected to the $V_{uc}$. 

\noindent\textbf{Modularizing Concern: Backtrack:}
Once the nodes at the output layer are channeled, we backtrack the concerned and unconcerned nodes to the previous layers. In this process, we remove the nodes that only participate in identifying the unconcerned classes. First, we discuss the backtracking approach to handle the dense layers and other non-dense layers, and then we describe how we can backtrack till the input to reduce the size of the module. In all approaches, we support the other layers, e.g., pooling, merge, flatten.

\begin{figure}[htp]
	\centering
	\includegraphics[, width=0.88\linewidth]{backtrack.pdf}
	\caption{Backtrack Through a Convolution Layer. }
	\label{fig:backtrack}
\end{figure}
\input{algodbp.tex}

\textbf{Modularizing Concern: Backtrack To Last Convolutional Layer (MC-BLC).}
%Furthermore, nodes at the $L_{d-1}$ layer that are only connected to the $V_{nc}$ are removed as these nodes do no participate in the classification task of the concerned output class.
Once we channel the output layer, we prune the network based on the inactive nodes at the dense layers. 
In a typical CNN model, either a \textit{Pooling} layer, \textit{Convolution} layer, or a \textit{Merge} layer will precede \textit{Dense} layers and the \textit{Flatten} layers 
In this approach, we leverage that information to backtrack through the \textit{Dense} layers (including \textit{Flatten} layer) to the last convolution layer(s) (based on the presence of \textit{Merge} layer or not) or the pooling layer. In this process, we identify the nodes that have edges $E=\left\{E_{ij}; i\in L_{d-1}, j\in L_{d}, j\in V_{l(uc)} \right\}$, where all the edges are only connected to the unconcerned nodes ($V_{uc}$) at the $d^{th}$ layer (line \ref{algo3:4}-\ref{algo3:10}). We start the backtracking process from the output layer and move through the dense layer. For each layer, we identify the nodes connected to the unconcerned nodes in the following layer and remove them from the model. Also, we tag the removed nodes as the unconcerned nodes for that layer. To identify the nodes that strongly contribute to the unconcerned node, we introduce a constant ($\delta$) to verify the value associated with the node. Based on the experimental evaluation, we used $\delta=0.5$. Then, we backtrack the nodes at the layer preceding the output layer is identified at line \ref{algo3:11}-\ref{algo3:17}. Finally, we backtrack to the flatten layer. In a traditional CNN model for image classification, the flatten layer is preceded by a pooling layer, or a merge layer, or a convolutional layer. 
If the preceding layer is a convolution layer, we update the mapping (as discussed in \S\ref{subsec:cl}) for that particular convolutional layer. Since the convolution layer's output is directly reshaped into the flatten layer, there is a one-to-one relationship between the two layers. If the preceding layer is a pooling layer, then there will be $X^2$ (X is the pool size) inactive nodes at the pooling layer for one inactive node at the flatten layer. If the preceding layer is a merge layer, then the convolution layers that are merged will be updated. 

%In Algo. \ref{algo:cmdbb}, we first backtrack through the dense layer to reach the flatten layer and identify the inactive nodes. From line \ref{algo3:4}-\ref{algo3:10}, all the nodes positively contribute towards the non-dominant node and negatively contribute towards the dominant node at the output layer have been identified. To identify the nodes that strongly contribute to the non-dominant node, we introduce a constant ($\delta$) to verify the value associated with the node. based on the experimental evaluation, we used $\delta=0.5$. Then, we backtrack the nodes at the layer preceding the output layer is identified at line \ref{algo3:11}-\ref{algo3:17}. Once we identify the nodes at the flatten layer, one of the three things can happen: 1) if the preceding layer of the flatten layer is a \conv layer, we update the map for the \conv layer. Since the convolution layer's output is directly reshaped into the flatten layer, there is a one-to-one relationship between the position of the nodes from the two layers. 2) if the preceding layer is an \textit{Pooling} layer, then for $pool_{size}^2$ inactive nodes at the flatten layer, there will be one node at \textit{Pooling} layer will be turned off. Based on the pooling layer principle, $pool_{size}^2$ nodes are converted into one node. The third possibility is the preceding layer is an \textit{Add} layer. Then, the maps correspond to the \conv layers that are merged will be updated. 
%\input{algodbp.tex}
\textbf{Modularizing Concern: Backtrack To Input (MC-BI).}
In the previous approach, we can only backtrack from the output layer to the last convolution layer. However, we cannot backtrack through the convolution layer. In a convolution layer, the input nodes cannot be directly mapped with the output nodes. For instance, in Figure \ref{fig:backtrack}, the input image shown on the left side is turned into the image shown in the middle, which is after adding the paddings (for this example, we choose \textit{Valid} padding). In the output, the nodes on the top left corner for both arrays will be produced by the first sliding window (blue box) from each array shown in the middle. So, for mapping, a node in the output on the right side of the image, at least 4 (in this example, we chose the sliding window size to be 2x2) nodes can be mapped. Those four individual nodes are also mapped with other nodes in the output. The black-colored node in the middle is a part of two sliding windows (the blue box and the orange box). To remove irrelevant nodes from the convolution layer, we take a two-pass approach. First, we store the position of the nodes in each sliding window with the nodes in the output (forward pass). 
During the forward pass, we store the mapping $M=\left\{(V_i, V_j) ; V_j=f(V_i, W, B)\right\}$, where $f$ denotes the convolution operation. During the backward pass, we remove the nodes.
\input{algobp.tex}
% In Algo. \ref{algo:cmfb}, we describe the step to do the mapping. From line \ref{algo4:1}-\ref{algo4:10}, the forward pass has been described. In the forward pass, we store the mapping between the sliding window and output nodes. In order to denote the position of the sliding window, we mark each node with a unique number (line \ref{algo4:4}-\ref{algo4:5}) before adding the padding. For padding, the nodes are marked as ``0'' as they are not present in the input of the \conv layer. Then for each output node, the input nodes are stored in a list. In the process, we define an operation named \texttt{sw} that computes the sliding windows from the input the weight $W$, padding $pad$, and stride. Since we use the similar implementation that \keras has, we do not show a detailed description. Furthermore, we compute the backward propagation based on the mapping found in the forward propagation. In the input, we have $preceeding\_layer$, $deactive\_map$, $depth$ that represents the type of the layer that precedes the current convolution layer, the list of inactive nodes found using the approach described in the \S\ref{subsec:challenges}, and the position of the \conv in the network. First, we compute the mapping with the input and the output nodes at line \ref{algo4:12}. 
%Then, we scan through the inactivate nodes in the output and identify if they match the pattern illustrated in Figure \ref{fig:backtrack}. 
%For each input node, we find all the output nodes generated from the particular input node. 


In Algo. \ref{algo:cmfb}, we describe the step to do the mapping. From line \ref{algo4:1}-\ref{algo4:10}, the forward pass has been described. In the forward pass, we store the mapping between the sliding window and output nodes. In order to denote the position of the sliding window, we mark each node with a unique number (line \ref{algo4:4}-\ref{algo4:5}) before adding the padding. For padding, the nodes are marked as ``0'' as they are not present in the input of the \conv layer. Then for each output node, the input nodes are stored in a list. In this process, we define an operation named \texttt{sw} that computes the sliding windows from the weight $W$, padding $pad$, and stride. 
%Furthermore, we compute the backward propagation based on the mapping found in the forward propagation. In the input, we have $preceeding\_layer$, $deactive\_map$, $depth$ that represents the type of the layer that precedes the current convolution layer, the list of inactive nodes, and the position of the \conv in the network. 
Now, we compute the mapping with the input and the output nodes at line \ref{algo4:12}. Then, we separate the input and the output nodes at line \ref{algo4:13} and \ref{algo4:14}. We scan through the inactivate nodes in the output and identify if they match the pattern as illustrated in Figure~\ref{fig:backtrack}. We identify all the input nodes that are mapped with an output node and vice versa. We focus on searching nodes that are not part of the padding operation and remove the nodes marked with 0 at line \ref{algo4:18}. For each such input node, we find all the output nodes generated from the particular input node. If these output nodes are already in the deactivation node list, we add the input node to the deactivation list for the preceding convolution (output of the preceding convolution layer is the input of the next convolution layer). If the previous layer is an add layer, then the two convolution layers that are merged at the merge layer are updated with the changes. If the preceding layer is a pooling layer, the update is carried based on the pool size. 


\subsection{Continuous Learning}
\label{subsec:cl}
In the prior study, reusing modules that originated from different datasets involves non-trivial cost. Our intuition is that since the modules are originated from a different dataset, they still have some traits of the parent dataset. In fact, by applying the tangling identification approach, we deliberately add some unconcerned examples to learn the modules on how to distinguish between the concerned and the unconcerned examples. However, in the inter dataset scenarios, the unconcerned output classes are not the same. To solve this problem, we propose a continuous learning-based approach. In deep learning, continuous learning~\citeauthor{collobert2008unified}~\cite{collobert2008unified} has been widely applied. In Figure \ref{fig:cl}, we illustrate a reuse scenario, where module F is originated from dataset 1 and module 2 is originated from dataset 2. Dataset 1 represents a set of English letters (A-G), and applying decomposition creates modules for each output class. Similarly, dataset 2 represents a set of English digits (1-7), and decomposition creates seven modules, each for one output class. When module F and module 2 are reused in a scenario, based on the prior work, each input belongs to 2, and F will be given as input to the composition of the decomposed modules. However, due to the parent dataset traits, module 2 can recognize itself but does not know how to distinguish from any input belonging to the output class F. To learn the concerned output classes in this scenario, we take the unconcerned section of the dataset. For instance, for module F, the unconcerned output class will be output class 2 from dataset 2. We take the examples from output class 2 from dataset 2 and update module F by removing the nodes responsible for detecting the output class 2. We do the same for module 2, where we remove the nodes responsible for recognizing output class F from dataset 1. Finally, the modified modules are ready to be reused.
\begin{figure}
	\centering
	\includegraphics[, width=0.84\linewidth]{CL.pdf}
	\caption{Continuos Learning. }
	\label{fig:cl}
\end{figure}
%
%\subsection{Continuous Learning.}
%\label{subsec:cl}
%\begin{figure}
%	\centering
%	\includegraphics[, width=1\linewidth]{CL.pdf}
%	\caption{Continuous Learning. }
%	\label{fig:cl}
%	\vspace{-10pt}
%\end{figure}
%%In the prior study, reusing and replacing the modules when the modules are originated from a different dataset (inter dataset) involves cost. 
%To solve this problem, we propose a continuous learning-based~\cite{collobert2008unified}  approach. 
%%In deep learning, continuous learning~\cite{collobert2008unified} has been widely applied in the natural language processing domain, where a pre-trained model is retrained with a different dataset. 
%In Figure \ref{fig:cl}, we illustrate a reuse scenario, where module F is originated from dataset 1 and module 2 is originated from dataset 2. Dataset 1 represents a set of English letters (A-G), and we decompose modules for each output class. Similarly, dataset 2 represents a set of English digits (1-7), and decomposition creates seven modules. When module F and module 2 are reused in a scenario, each input belongs to 2, and F will be given as input to the composition of the decomposed modules. However, due to the parent dataset traits, module 2 can recognize itself but does not know how to distinguish from any input belonging to the output class F. To learn the non-concerned output classes in this scenario, we take the non-concerned section of the dataset. For instance, for module F, the non-concerned output class will be output class 2 from dataset 2. We take the examples from output class 2 from dataset 2 and retrain module F by removing the nodes responsible for detecting the output class 2, from our mapping. We do the same for module 2, where we remove the nodes responsible for output class F from dataset 1. Finally, the modified modules are used for the reuse scenarios.

==> dataset.tex <==
\section{Dataset and Model Descriptions}
\paragraph{Datasets} We evaluate our proposed approach based on three widely used and well-vetted datasets.

\noindent\textbf{CIFAR-10~\cite{krizhevsky2009learning}:} This dataset comprises of 3-D images of different objects. It has 10 output classes, and the dataset is divided into training and testing datasets. The training dataset has 50,000 images and the testing dataset has 10,000 images. The number of examples for each class is equally distributed. The output classes are airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. Each of the images is of size (32, 32, 3), where the length, width, and color channels are 32, 32 pixels, and three dimensions, respectively.

\noindent\textbf{CIFAR-100~\cite{krizhevsky2009learning}:} This dataset has 100 output classes. This is widely used to evaluate CNN-based studies due to the complexity of the dataset. Here, there are 50,000 training images and 10,000 testing images. There are 20 different types of images in this dataset, and for each type, there are 5 varieties of images are there. For instance, one of twenty superclasses is the aquatic animal, and within that class, we have beaver, dolphin, otter, seal, and whale. The image size is similar to the CIFAR-10.

\noindent\textbf{ImageNet-200~\cite{deng2009imagenet}:} This dataset is very popular and widely use to measure the scalability of CNN-based applications. Unlike the previous two datasets, the total number of output classes is 200. ImageNet dataset has been designed to help the computer vision-related task in machine learning. This dataset has 80,000+ nouns (name of the class), and for each class, there are at least 500 images associated with it. This dataset has been used in training models in real-life scenarios. However, due to the complexity of the dataset, a smaller dataset specially intended for research purposes with similar complexity has been made public. This dataset (ImageNet-tiny) comprises 200 types of images. The training dataset has 100000 images, and the testing has 10000 images. There are 3 different variations of the dataset, where the length and width of the images are 224, 64, and 32. In our experiments, we used the 64 version of the dataset to reduce the time-complexity of training such networks and have an experimental dataset that is different from CIFAR-10 and CIFAR-100 in terms of the image size. 
\paragraph{Models} In this study, we used the ResNet models to evaluate our proposed approach. There are multiple blocks present in a ResNet model, and each block consists of convolution, add, and activation layers. There are two versions of ResNet, the original version, where there is a stack of convolution, add, and batch normalization layers are put together to form a residual block, and finally, those residual blocks build the network. In the second version, the residual block is modified to form a bottleneck layer with convolution, add, and batch normalization. We performed our evaluation against the first version of the network for simplicity and to reduce the training time and resources. Each such version can either have a batch normalization layer or not, as described in the original paper. Since batch normalization is only used to train and does not participate in the prediction, we chose the model without batch normalization to reduce the training time as some of our experiments include training models multiple times. We used ResNet-20, ResNet-32, and ResNet-56, where 3, 5, and 9 residual blocks are present with 21, 33, and 57 convolution layers, respectively. The accuracy reported in this study is different from the original paper because we re-trained the model from scratch with 200 epochs.

The code can be accessed at.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
\begin{figure*}[!ht]
	\includegraphics[, width=1\linewidth]{overview.pdf}
	\caption{How Decomposing a Convolution Neural Network can Help Solving a Real-life Problem.}
	\label{fig:overview}
\end{figure*}
Decomposing a convolutional neural network into modules can help to achieve various real-life scenarios. Because of the complex architecture and the massive size, retraining a model from scratch is not always feasible. Instead of building a new model, we propose utilizing parts from the already trained model and reusing or replacing them based on different scenarios. First, we describe one such requirement, where replacing a section of the model (module) with another (module) can be done with no or little retraining. Then, we describe how reusing these modules can be done.

In Figure \ref{fig:overview}, we have shown a real-life example, where Google Photo App tagged a black woman as a gorilla. To resolve this issue, Google has decided to remove the output class ``Gorilla'' by suppressing the output label. In fact, they have suppressed labels for ``Chimpanzee'', ``Monkey'', ``Chimp'', etc~\cite{verge}., from the output of the convolutional neural network. Though the problem can be temporarily solved by suppressing the output label, to fix the model, one needs to retrain from scratch, which requires both high-computational and time-related resources. Instead of the prior approach, we propose three different solutions that reuse and replace modules from the trained model. We will discuss each of such approaches and their pros and cons and illustrate how retraining the model can be avoided. 

First, we decompose the faulty convolution neural network into modules for each output class. For instance, we have one module for each output class that classifies whether an input belongs to the output class, for which the module has been created, or not. In this example, our goal is to replace the faulty part or module responsible for classifying gorilla with a working module for the same. If we have another working model that is either trained with the same dataset or a subset of the dataset, we will decompose that working model into modules. The working model needs to have the gorilla and person output label, and that model should not exhibit the behavior present in the faulty model. Then, we can replace the faulty gorilla module with the working gorilla module, and a composed version of the decomposed modules can be sent to production. However, the drawback of this approach is the availability of such models. Training a model with a large dataset needs heavy computational resources and a non-trivial amount of time.

Second, we decompose the faulty model into modules. Moreover, we train a new model with a person and gorilla and validate that the trained model does not demonstrate faulty behavior. We decompose the newly trained model into two modules and replace the faulty gorilla module with the new decomposed gorilla module. In this scenario, decomposition can not alone solve the problem. However, the decomposition bundled with the traditional training could help in this situation. Also, training the small model requires less resources.

Third, we decompose the faulty model into modules and remove the gorilla module from the collection. In this scenario, there is no cost of retraining involved. However, using this approach, the actual problem of faulty classification has not been addressed. This solution is similar to what Google proposed, but instead of suppressing the label, we remove the module. The pros in this situation are that for other primates (``Chimpanzee'', ``Monkey'', ``Chimp'', etc.), we can remove the modules easily, whereas, for the other two techniques, we need to have models with those output classes or train a small network for them. 

We can also reuse the person and gorilla module from a working model without the faulty behavior and predict any input classified as a person or gorilla using the faulty model to verify it further. Here, instead of replacing the faulty parts, we reuse modules and add another verification with them.
